Earth+: on-board satellite imagery compression leveraging historical earth observations

With the increasing deployment of earth observation satellite constellations, the downlink (satellite-to-ground) capacity often limits the freshness, quality, and coverage of the imagery data available to applications on the ground. To overcome the downlink limitation, we present Earth+, a new satellite imagery compression system that, instead of compressing each image individually, pinpoints and downloads only recent imagery changes with respect to the history reference images. To minimize the amount of changes, it is critical to make reference images as fresh as possible. Earth+ enables each satellite to choose fresh reference images from not only its own history images but also past images of other satellites from an entire satellite constellation. To share reference images across satellites, Earth+ utilizes the limited capacity of the existing uplink (ground-to-satellite) by judiciously selecting and compressing reference images while still allowing accurate change detection. In short, Earth+ is the first to make reference-based compression efficient, by enabling constellation-wide sharing of fresh reference images across satellites. Our evaluation shows that Earth+ can reduce the downlink usage by a factor of 3.3 compared to state-of-the-art on-board image compression techniques while not sacrificing image quality, or using more on-board computing or storage resources, or more uplink bandwidth than currently available.

==> tex-files/intro-v2.tex <==
%!TEX root = ../paper.tex
%!TEX spellcheck = en_US


\section{Introduction}



% Satellite imagery, and its corresponding applications, are growing rapidly.
Fresh and high-quality satellite imagery is key to many applications. 
With more satellites capturing images at higher resolutions, satellite imagery has promised to transform
% The increased availability of satellite images with high resolution and short revisit time have enabled 
applications from digital agriculture ~\cite{mulla2013twenty, hank2019spaceborne,planet-digital-agriculture,digital-agriculture1}, environmental monitoring~\cite{manfreda2018use, tucker2000strategies, tralli2005satellite, cunjian2001extracting,environment-monitoring1}, to automatic road detection~\cite{kopsiaftis2015vehicle, van2018spacenet,automatic-road-detection} and many more.
% However, limited by the downlink capacity, the satellite imagery captured by the satellite cannot be fully downloaded by the satellite.
However, the reality is that most satellite imagery data are not received on the ground due to {\em limited downlink capacity} (satellite-to-ground).
% However, bottlenecked by the downlink capacity, 
By a recent estimate, only 2\% of the total image data observed by each satellite are downloaded to the ground~\cite{kodan}.
%Despite efforts to expand the downlink capacity, they incur high costs to deploy more ground stations and reserve more bandwidth.
%As a result, downlink capacity remains a bottleneck, which severely limits the coverage, fidelity, and freshness of images available to applications.


%Different satellite constellations tackle this downlink bottleneck differently.
%% depending on their missions. 
%%Facing this downlink bottleneck, there are two types of satellite \textit{constellations} that handle this bottleneck in different ways.
%% \peder{the ground can download?}
%Mission-based satellite constellations~\cite{kodan,oec} focus on a small fraction of 
%%The first type of satellite constellations~\cite{kodan,oec} are built with a mission that focuses on a small subset of 
%geographical locations that are pre-determined by certain applications. 

\shadi{This part breaks the flow. Need to paint the big picture first}
\shadi{An alternative: talk about the large data in LEO constellation and the gap between data captured and downlinked. }
Many previous efforts tackle this downlink bottleneck in the context of mission-based satellite constellations~\cite{kodan,oec}, which focus on a small fraction of geographical locations pre-determined by the specific applications. 
For instance, Biomass mission~\cite{biomass} targets forest areas and runs mission-specific filters (\eg forest filter) to collect only relevant images from the satellites. 
% These satellites run mission-specific filters (\eg forest filter for Biomass mission~\cite{??}), so the images of the selected areas can be downloaded with existing downlink capacity.
%As a result, these satellites run mission-specific filters (\eg forest filter for Biomass mission) to filter out a large percentage of the areas on the earth (\eg about 91\% earth surfaces can be filtered out~\cite{forest-area,ocean-area} using forest filter), so the downlink capacity is sufficient for downloading the data of remaining areas.
However, these mission-based satellites may filter out data useful for other applications.
For instance, a forest filter can filter out about 91\% earth surfaces~\cite{forest-area,ocean-area}, \eg agricultural areas which can be crucial for crop monitoring.


% Rather than improving the filtering on mission-based satellites, 
Instead, we focus on
% in this work is to enable better on-board image compression for 
{\em general-purpose} earth-observation satellites,\footnote{The earth-observation satellites are different from the low-earth orbital (LEO) satellites, such as Starlink, designed for Internet connections.} such as Sentinel-2~\cite{sentinel-2}, PlanetScope~\cite{planet}, Landsat~\cite{landsat}, whose mission is to download as much earth imagery data as possible, with high coverage, freshness, and fidelity.
%Many satellite constellations (\eg Sentinel-2~\cite{sentinel-2}, PlanetScope~\cite{planet}, Landsat~\cite{landsat}) are general-purpose and aim to download all earth imagery data.
Today, these satellites must compress the imagery data aggressively before sending them to the ground, causing low fidelity (resolution), freshness, or coverage of the downloaded images. 
%%The second type of satellite constellations are designed with a general-purpose mission that instead aims to download data all over the earth (\eg Sentinel-2~\cite{sentinel-2}, PlanetScope~\cite{planet}, Landsat~\cite{landsat}).
%This type of satellites handle the downlink bottleneck in two ways. 
%% either by downloading low-resolution satellite imagery or augmenting the downlink capacity (\eg Sentinel-2, PlanetScope).
%% Both choices are not ideal.
%The first way is to download low-resolution satellite imageries.
For example, MODIS constellation~\cite{MODIS} downloads images at low fidelity, with a ground sample distance (GSD) of 250m (defined as the distance between the centers of neighboring pixels), which is inadequate for 
% However, such low-resolution images do not suffice for 
applications, such as crop growth monitoring, precision agriculture, urban expansion analysis, and 3D city monitoring, which demand a GSD of 5-30m or lower~\cite{application-GSD}.
There are also limited efforts to upgrade the physical infrastructure on both the ground station and the satellites to increase the bandwidth capacity~\cite{planet,sentinel-2,kodan}.
% , or applications like 3D city monitoring and precision agriculture (which require a GSD of 1-5m~\cite{application-GSD}).
% Alternatively, satellite imagery providers may expand the downlink capacity by building more ground stations or parallelizing the download across satellites in a constellation~\cite{planet,sentinel-2,kodan}.
Yet, a large fraction of images (\textit{e.g.} about 70\% areas
% \footnote{The majority of ocean areas is not observed in Sentinel-2~\cite{sentinel-2-ocean}, which corresponds to about 70\% areas on the earth.} 
in Sentinel-2~\cite{sentinel-2})
% \jc{can we not mention ocean; just say the \%?}) 
still are not downloaded.
% \shadi{maybe talk about the large scale that planet generates with numbers.}

%\jc{i removed the cost argument agains expanding capacity because it's been discussed in the 2nd paragraph. Kuntai, please move the text there if you see appropriate.}
% \jc{The cost argument seems to be misplaced here: with their current DL capacity, is Sentinel-2 or PlanetScope already capable of downloading everything at a desirable quality level? If they already do, then why bother? If they have already deployed enough capacity, saving the cost for them seems like weaker position. But I guess even with the new DL capacity, the bottleneck still remains (which is a stronger position), right? If so, let's don't put the cost argument here.}
% \jc{Sending more satellites increases the DL capacity? Thßis seems counterintuitive. Won't having more satellites produce more images instead?}

%Rather than improving the filtering on mission-based satellites, the focus of this work is to enable better on-board image compression for general-purpose satellites to download more images at better fidelity under limited downlink capacity.\footnote{We want to clarify that this work is orthogonal to the recent proposals to improve the low-earth orbital (LEO) satellite constellations that are designed for Internet connections, such as Starlink.}


%The research focus of this paper, is to handle the downlink bottleneck of general-purpose satellite constellations by improving the on-board satellite image compression, so that existing general-purpose satellites can download more images to the ground station, and future general-purpose satellite constellations can be built and maintained with less cost.


%\jc{the next 5-6 paragraphs need to be tightened}

% \jc{below is a compact version of the four paragraphs. i commented the old text for your reference.}



% To let satellites send more images to the ground at a higher fidelity under limited downlink capacity, we set out to improve on-board satellite imagery compression.
% Though there is a long history of ground-based satellite image compression (\eg~\cite{satroi,virtual-background,change-encoding}), on-board image compression, where compresses images before sending it to the ground uses only information a satellite can access locally, also has recently gained attention. 
% We follow the general approach of {\em change-based encoding}~\cite{satroi,virtual-background}, where 
\shadi{need to point out compression as a good way to bridge the gap first}
In this paper, we improve on-board satellite image compression, by taking the emerging approach of {\em change-based encoding}~\cite{satroi,virtual-background}. 
\shadi{need to highlight that images rarely change}
Unlike whole-image compression widely deployed on satellites, change-based encoding compares each new image with a {\em reference} image captured previously by the satellite at the same location and only compresses and sends the regions that have changed since the reference was taken. 


Unfortunately, directly applying change-based encoding to on-board image compression is inefficient.
Change-based encoding works well when the reference images are {\em fresh, cloud-free} (\S\ref{subsec:up-to-date-reference}). 
% This is likely true for ground-based satellite image compression (\eg~\cite{satroi,virtual-background,satroi-2}) since the ground can access the history images from multiple satellites, but 
However, the satellite only has access to its own historical images, making it difficult to get fresh and cloud-free reference images.
To put it in perspective, a satellite typically photographs the same location every 10 days~\cite{sentinel-2-revisit}, and this image is likely cloudy as 2/3 of the earth's surface is covered by cloud at any time~\cite{cloud-coverage}.
As a result, the satellite can only obtain a cloud-free image once every \fillme days.
% \shadi{what are longer numbers?}
With such reference staleness, most regions might have changed since the reference and thus must be compressed, which negates the benefit of change-based encoding. 
To make it worse, if a reference image is (partially) covered by cloud, one must go back further in time to find a cloud-free reference image with an even longer staleness. 
\shadi{give numbers on how often this happens.}
In short, the compression efficiency of current change-based encoding is limited by {\em local} information available to a satellite.
% If the reference image is stale, \eg for a few days, most regions in the reference image might have already changed since then and have to be compressed, which negates the benefit of change-based encoding. 
% Similarly, if clouds cover a region in the reference image, the pixels of the region in the new image will be counted as changed and will be downloaded (unless it is covered by clouds again).



% Even though change-based encoding is well-suited for ground-based satellite image compression (\eg~\cite{??}) since the reference can be any image from any satellites, each satellite often does not have access to a fresh and cloud-free reference image locally. 
% Instead, each satellite takes a photo of the same location every 10 days or even longer~\cite{sentinel-2-revisit}.
% This means that the reference images have a long stale and many regions have changed between two visits, causing many regions to be downloaded.
% To make it worse, if a reference image is (partially) covered by cloud, one must go back further in history to find a cloud-free reference, with an even higher staleness. 
% In short, the compression efficiency of current change-based encoding is limited by {\em local} information available to a satellite.

% \jc{end of the new text}


\begin{comment}

This paper aims to let satellites send more images to the ground at a higher fidelity under limited downlink capacity by improving on-board satellite imagery compression.
There has been active research on satellite imagery compression (\eg~\cite{satroi,virtual-background,change-encoding}), with a basic observation that 
%Prior work~\cite{satroi,virtual-background,change-encoding} identifies an opportunity to further compress satellite imagery: 
the geographical content is mostly unchanged between two consecutive satellite visits.
This observation inspires \textit{change-based encoding}:
one can use a previous image from prior satellite visits at the same terrestrial location as the reference to identify the changed regions in the current satellite visit and focus the encoding only on the changed regions.
%We call this approach \textit{change-based encoding.}
Using such change-based encoding, the satellite only needs to download ??\% of the geographical areas in average, a ??x compression (see \S\ref{??} for the details of our measurement).\kt{need detailed numbers here}
% \item
% First type of work: existing satellite imagery encoders. Cons: areas that are not changed also need to be downloaded. \kt{Merge para 3.}

Though promising, such change-based encoding heavily relies on \textit{up-to-date, cloud-free} reference images as reference. %in order to significantly save the usage of downlink.
For instance, in an agriculture application, if the reference image is (partly) covered by clouds,  it will be impossible to determine if some changes have occurred to the pixels of the current image that overlap with the clouds, and as result the satellites may encode and send more pixels than necessary.
Similarly, if the reference image is out-of-date, the satellite may redundantly send out changes that are already observed by a recently-captured imagery at the same location, leading to extra downlink usage.

%\jc{two key ideas: (1) use more satellites to get up-to-date cloud free, (2) how to best leverage uplinks}

%For example, in agriculture areas, the color of the soil changes significantly after raining.
%Thus, all soil areas will be counted as change and be downloaded if we use a reference image before the rain happens.
%Empirically, we measure the amount of changes with respect to the staleness of the reference image, and found that XXX.

Thus, a key challenge of change-based encoding is 
%As a result, the challenge of implementing such change-based encoding is 
\textit{how to obtain fresh, cloud-free reference images on-board}.
One typical solution is to maintain an on-board repository that contains one reference image for every terrestrial region, and update this image when a new cloud-free image is observed by the satellite. 
The problem is that even if there is enough on-board storage to store these reference images, the last cloud-free images might be out-of-date in many regions, because each satellite revisits the same terrestrial location only once about every 10 days, and a cloud-free image may not be captured every time it visits a region.



In short, the compression efficiency of current change-based encoding is bounded by {\em local information available to a satellite}.

\end{comment}

\begin{comment}

Prior work~\cite{satroi,virtual-background,change-encoding} stores the reference image on-board (with sufficient compression to fit into on-board storage) and update the reference images when a new cloud-free image is observed.
However, the reference image of this approach is stale due to two reasons.
First, as the satellite revisits the same location once every 10 days~\cite{sentinel-2-revisit}, the satellite can only refresh the reference image for that location once every 10 days.
Second, when a new image is observed, that image can be cloudy and cannot be used as future reference, thus further postpone the updating of the reference image.
% Facing this design question, prior work~\cite{satroi,virtual-background} uses the on-board storage to store the reference images for all geographical locations are stored on the satellite.
% However, to store reference images for all locations, the reference images need to be aggressively compressed with a compression rate larger than 400, which forces the satellite to download more than half of the areas in order to cover all the changes (see detailed measurements in \S\ref{??}).\peder{missing reference}

\end{comment}






% First, the satellite does not have sufficient on-board computing power to handle the dynamics above the ground, like clouds and shadows. 
% Even though these areas can be efficiently skipped, 
% Second, the satellite does not have sufficient storage to store a reference image for every area that the satellite visits, as this requires storing ??PB of the data on the satellite, ??x larger than the satellite disk capacity even after compressing the images by ???x.
% \kt{Give people a sense of how expensive it is to expand the on-satellite storage.}
% Even if the satellite \textit{could} have a disk with almost infinite storage that can save the latest historical images of all regions, XXX.

% \kt{Need to confirm with Peder why the satellites cannot have disks with super large capacity} \jc{while you check with peder, can we claim something like ``even if a satellite does store the latest history images of all regions and uses them to detect only changes, its still not efficient since the more recent the ref image is the better, and each region is photoed by the same satellite only once every xxx days but will be by {\em some} satellite every xxx hours?''}

% \kt{I am thinking of also mentioning the reason that the satellite does not have enough compute to handle clouds. Pros: }
% \item 
% \kt{New reality: uplink, on-board computing}
% \kt{New reality inspires a new pipeline}
% \kt{Realize this potential, key design questions (reference image, configuration, cloud/illumination}
% \kt{Why answering these questions are not trivial?}

% We observe a new trend on the satellite: the \textit{on-board computing} on the satellite becomes more abundant, and the \textit{uplink capacity} from the ground station to the satellite is becoming larger and larger.
% For example, \kt{a list of data to instantiate this point.}

% \jc{we should emphasize that the ref image can be from {\em any} satellite that has flown by the location recently} 
% \jc{we should highlight that our design enables each satellite to virtually have access to images taken by {\em all} satellites to compress each image.}
% To store reference images under limited on-board storage, our insight is that: for a given geographical location, its corresponding reference image only needs to be on-board when the satellite flies by that location.
% In other word, instead of saving the reference images for all locations, the satellite only need to save the reference images for \textit{a small subset} of locations that the satellite is going to fly by.

% Based on this insight, we advocate for a design that the ground upload the reference image to the satellite for the locations that the satellite will visit before next ground contact.


\kt{I am now rewriting this part.}
To overcome this limitation, we propose \textit{constellation-wide change-based encoding}, where the satellite can pick \textit{any images observed by the whole constellation} as the reference.
% Figure~\ref{fig:earth_plus}
% two-fold.
With constellations typically containing many satellites (\eg more than 130 satellites in DOVEs constellation~\cite{planet}), each location will be photoed frequently (\eg once every few hours in DOVEs constellation) by one of the satellites.
This significantly improves the freshness of cloud-free reference images. \kt{Need some numbers here}.


The key design question of such constellation-wide change-based encoding is \textit{on-board the satellite, how to obtain reference images that are from other satellites in the constellation}.
We leverage the \textit{uplinks} to {\em upload} fresh and cloud-free reference images from the ground to the satellites (illustrated in Figure~\ref{fig:highlevel}).
An alternative design is to leverage inter-satellite links to stream images from one satellite to another.
However, this approach is less preferable, since the satellite does not have sufficient compute to determine if a image is cloud-free (and thus can be reference image) or not.
Moreover, current earth observation satellites do not have such inter-satellite link readily available.
% \footnote{Though direct inter-satellite links could be used to share images across satellites, they are not readily available in most earth-observing satellites.}
% Our vision, therefore, is to use the uplinks to enable each satellite to potentially access all images transmitted to the ground by {\em any} satellite in an entire constellation.


% Second, uplink is commonly available in earth observation satellites, because the ground needs to send control messages to the satellite.
% In contrast, one can also leverage inter-satellite link to access images from other satellites, but such inter-satellite link is not readily available in existing earth observation satellites.



% (the link from the ground to the satellite) to update the reference images on the satellite, so that each reference image only needs to be on-board  the storage demand on the satellite. Concretely, we let the satellite cache the reference images for \textit{a small subset} of locations, and \textit{timely update} this cache to make sure the satellite have access to future locations.
% \kt{A figure to contrast prior design and our design}
% Then, the satellite captures the image for that location, compares this image with the reference image, and only stores the changed areas.
% Then the satellite captures the image of this location, saves the parts that differ from the reference image, and deletes the reference images after use. 
% Compared to prior design that stores reference images for all geographical locations, the advantage of our design is two-fold:
% \begin{packeditemize}
%     \item Our design enables the satellite to use the images from \textit{other satellites} as the reference.
%     access higher-quality reference images\kt{quantify}, which allows the satellite to download only 10\% areas while still covering all changes.
%     \item Further, this design allows the satellite to access a more up-to-date reference image by using the images from \textit{other satellites} as the reference. 
%     To show the concrete potential, we perform a measurement in \S\ref{??} \kt{fill in more details here}
% \end{packeditemize}


% First, this design increases the potential of change-based encoding. By streaming the reference image up to the satellite, the satellite can access images from \textit{other satellites}, enabling it to stream a more up-to-date reference image to the satellite.
% First, this design allows the ground to streaming the images from \textit{other satellites} as the reference. The satellite can thus obtain a more up-to-date reference image and download much fewer changed areas compared to using the images from the satellite itself as the reference image.
% df downloaded while still maintaining  obtain a more up-to-date reference image, thus the satellite can encode much less areas 
% uploading the reference images from the ground, the satellite virtually has access to the images taken by \textit{all} satellites, which provides much higher compression capability than ABC.

% Second, this design significantly reduces the resource demand of performing change-based encoding on the satellite, in terms of both storage and on-board computing power.
% This is because the satellite can immediately delete the reference image of one location after it finishes visiting that location.
% This reduces the number of reference images that the satellite needs to store from ??? to ???, a ???x reduction.
% Also, the ground can customize the cloud detector and the change detector based on different geographical locations and other satellites. As a result, the satellite can perform accurate cloud detection using a cheap decision-tree-based cloud detector (rather than an expensive neural-network-based cloud detector~\cite{??}).
% Second, this design reduces the storage requirements on the satellite by ????x compared to storing all reference images on the satellite, making it possible to fully leverage the potential of only downloading changed areas under limited satellite storage space.


% \jc{i'd seriously downplay the first question. it's more like an ml question. i understand you spent a lot of time on it, and it's important to make it work, but it's not really relevant to "how to leverage the big pool of history images", which is the key up until this point in the story}
% \jc{this sounds more like why (3) is challenging, not a design question..}
% \jc{i'd put this upfront. this is the key challenge.}
% To realize this potential, we list three design questions are:
% \begin{enumerate}
%     \item How to detect changes on the satellite, given the varying cloud and illumination conditions? 
%     \item How to obtain the best image quality (in terms of PSNR) under limited satellite computation power, storage, and limited link capacity between the satellite and the ground station?
%     \item How to develop a mechanism to avoid letting the error (introduced by not downloading some of the areas) propagate. 
%     \item How to select reference images? 
% \end{enumerate}


%To instantiate the design above, we propose \name, the first system that improves satellite imagery compression by leveraging historical earth observations. 



% The major practical challenge of \name is that the total file size of reference images significantly exceeds the limited uplink capacity (only 250kbps~\cite{dove-uplink-downlink} for DOVEs constellation) of earth observation satellites.
% To handle the limited uplink, \name stores the reference images on-board and update a small subset of reference images (where the satellite will fly-by before next ground contact) during each ground contact.
% We illustrate this design in Figure~\ref{fig:uplink-design}.


% Compared to prior solutions that encode and download observed images in their entirety, \name stores the reference images on-board without requiring more on-board storage due to the following two reasons:
% \begin{packeditemize}
%     \item Compared to current satellites that stores every pixel of the captured images on-board, \name only saves changed pixels on-board, squeezing out limited storage space for \name to store reference images.
%     \item Even though the reference images need to be heavily compressed to fit into this limited storage space, the changes can still be accurately detected and downloaded (with marginal cost of slightly downloading more areas than necessary --- we will quantify this overhead in \S XX).
% \end{packeditemize}

% Besides the compression of the reference images, \name further cut down the usage of uplink using the following two optimizations:
% \begin{packeditemize}
%     \item During each ground contact, the ground only need to update references for those locations that the satellite will fly-by before the next ground contact, which is $160\times$ smaller than the total number of locations.
%     \item  The ground only needs to upload the \textit{difference} between the on-board reference images and the reference images to be uploaded. This can significantly reduce the amount of data need to be transferred, as the reference images to be uploaded are the same as the on-board reference images on most of the geographical areas.
% \end{packeditemize}
% With these two optimizations, \name is able to update the corresponding reference image before capturing a new image.

\begin{figure}[t!]
    \centering
    \hspace*{-0.5cm} 
    \includegraphics[width=0.53\textwidth]{figures/highlevel-contrast-intro.pdf}
    % \begin{subfigure}[b]{0.99\columnwidth}
    %     \centering
    %     \includegraphics[width=0.8\textwidth]{figures/highlevel-contrast-without-uplink.pdf}
    %     \caption{Traditional workflow of downloading satellite imagery.}
    %     \label{fig:highlevel:no-uplink}
    % \end{subfigure}
    
    % \centering
    % \begin{subfigure}[b]{0.99\columnwidth}
    %     \centering
    %     \includegraphics[width=0.8\textwidth]{figures/highlevel-contrast-with-uplink.pdf}
    %     \caption{\name gathers reference from the entire constellation and use reference to further compress satellite imagery.}
    %     \label{fig:highlevel:no-uplink}
    % \end{subfigure}
    \tightcaption{Contrasting between traditional satellite imagery compression pipeline and our uplink-based imagery compression pipeline.
    In the traditional design shown in (a), the satellite compresses the imagery using local information on the satellite.
    However, in our design shown in (b), the satellite can refer to imagery from other satellites for better satellite imagery compression.
    }
    \label{fig:highlevel}
\end{figure}

The challenge of streaming reference images using uplink is that the uplinks have {\em much insufficient capacity} to upload many high-quality reference images. 
% Unlike communication satellites, 
The uplinks of earth-observing satellites have historically been used to send control messages between the ground and the satellites. 
For instance, the uplinks of DOVEs constellation have only 250kbps~\cite{dove-uplink-downlink}, which is 800$\times$ smaller than its downlink capacity.
%the primary challenge with \name is the substantial file size of reference images, which surpasses the limited uplink capacity (250kbps\cite{dove-uplink-downlink} for the DOVEs constellation) of earth observation satellites. 


To address this challenge, we present \name. \name uses several optimizations (\S\ref{sec:reference-uploading}) to significantly lower the uplink usage   without sacrificing the savings on the downlink usage. 
Here, we highlight two of them.
{\em (i)} First, \name uploads reference images at a low resolution (256$\times$ downsampling, width, and height) that still allows the satellites to identify most of the changed regions (\fillme$\times$\fillme blocks).
The intuition is that identifying which blocks contain terrestrial changes (\ie a binary classification),  requires much less information than pinpointing the exact value changes in each block. 
{\em (ii)} Second, \name also batches image updates across satellites to avoid repeated updates in frequently changing regions. 
Finally, these steps can surely cause some changed blocks not to be downloaded, and \name mitigates these ``false negatives'' by periodically downloading a whole image without using the reference images at a low frequency.







\begin{comment}
    


%To address this, \name retains reference images on-board and updates a subset corresponding to imminent trajectory of the satellite during each ground contact. This approach is depicted in Figure~\ref{fig:uplink-design}.
%
%Unlike traditional methods that download observed images in their entirety, \name stores reference images without requiring additional storage space. This is achieved by:
\begin{packeditemize}
% \item 
% % \textit{Reducing the resolution}
% \name leverages multiple ground stations and uploads the subset of reference images at only the locations to be visited by the satellite between two consecutive ground contacts. 
% Figure~\ref{fig:uplink-design} illustrates this idea. 
% \jc{i was adding the 160$\times$ number here, but it may seem too much a gain from a single optimization, and diminish the importance of other ideas. do you think so?}
%\item \name only saves the pixels that have changed, thus conserving space that can be allocated for reference images.
% \item Instead of updating the reference image every time before visiting a geographical location, \name only updates its reference image when \textit{other satellites} obtain a new \textit{cloud-free} reference image. 
% This reduces the frequency of updating the reference image by ??$\times$ (\S\ref{??}).
% This allows us to strike a balance between uploading fewer reference images on the uplinks and potentially downloading more detected changed regions on the downlinks.
%\item Compressing the reference images to fit within the storage constraints. Despite this compression, \name is capable of detecting and downloading over 99\% of the changes, with the cost that some unchanged areas may be downloaded (\S\ref{??} discuss this overhead in detail).
\item \name uploads reference images much lower resolution (128$\times$ downsampling, width and height).
Such low resolution still allows the satellite to detect changes.
This is because sdf.
%  because most of the changes on the ground is large-scale changes.
% For example, during harvesting season, a farm can change between two consecutive satellite visits.
Intuitively, many changes (though not all) on earth's surface are non-trivial changes on satellite images that can be detected by comparing them with a low quality reference image. 
For instance, \name is capable of detecting and downloading over 99\% of the changes, with the cost that some unchanged areas may be downloaded.
\end{packeditemize}
Taken together, these strategies enable \name to refresh the relevant reference images, despite the low uplink capacity.

\end{comment}

\begin{comment}
In addition to compressing reference images, \name further optimizes uplink usage in two ways:
\begin{packeditemize}
\item During each ground contact, only references for imminent satellite trajectories are updated, reducing the locations updated by a factor of $160\times$.
\item Only the \textit{difference} between on-board and new reference images is uploaded, reducing data transfer as most images remain largely unchanged from their previous upload.
\end{packeditemize}
\end{comment}
%prior to a new capture.



% To handle such limited uplink, \name amortize the uploading of the reference images across different ground contacts.
% Concretely, during each ground contact, \name uploads the reference images for a small subset of future locations, which the satellite will fly-by before next ground contact. \jc{Doesn't this mean reference images will be less up-to-date? It seems to defeat the previous claim that reference must be up-to-date, right?}
% Further, \name only streams the difference between the reference images to be  uploaded and the reference images on-board.
% With these two optimizations, \name is able to provide a new reference image everytime when the satellite captures a new image, without exceeding limited uplink bandwidth.

% \jc{I think it's necessary to bring up the insight that low-quality reference is enough for change-based encoding. Otherwise, because you need a reference in each location, the storage cost will be prohibitive.}



% \begin{packedenumerate}    
%     \item 
%     How to upload the reference images to the satellite, given the extremely limited uplink capacity (only 250kbps~\cite{dove-uplink-downlink})?
%     % \item 
%     % How to determine the policy of uploading reference images (\ie which locations should have their reference images uploaded in what quality), in a way that is aware of the varying uplink capacity (characterized in \S\ref{??}), while still allowing the satellite to access high-quality reference image?
%     \item 
%     How to detect changes under varying cloud condition (and also illumination condition) so that almost all changes can be detected without exceeding the computation capacity on-board?
% \end{packedenumerate}


% To upload reference images under limited uplink, \name only updates the difference between the reference images to be uploaded and the current reference images on-board.
% This significantly saves the am

% We further present implementation details of \name that allows \name to perform change detection under the dynamism of satellite imagery (including cloud and illumination difference between images).


% \kt{Feel free to skip this paragraph. I need more measurement to support it.}
% Another challenge of \name is to detect changes while fitting into the limited computation resource on the satellite.
% The change detection process is computationally expensive as it needs to  detect changes under varying cloud coverage condition, while accurately identifying clouds require running tens of layers of neural networks~\cite{change-encoding,cloud-net}.
% To reduce the computation cost of change detection process, our insight is that cheap algorithms (\textit{e.g.} decision-tree-based cloud detector and pixel-difference-based change detector) can already accurately predict changes on over XX\% of the geographical areas.
% % \jc{what does this cheap algorithm have to do with the use of uplinks?}
% As a result, \name runs cheap algorithms to detect changes, and download the changes together with the areas that the cheap algorithms are likely to produce errors.




% We proposes three techniques to address these challenges. \kt{need to fill the detail of these techniques}.
% \begin{packeditemize}
%     \item Obtaining the reference image $\rightarrow$ reference image stitching
%     \item Varying uplink condition $\rightarrow$ keep more images on the satellites to safeguard against potential ground disconnection
%     \item Change detection using limited resource $\rightarrow$ 1. perform coarse-grained cloud and change detection, using cheap algorithm. Insight: cheap algorithm may perform really bad in its application-specific metric, 2. using reference image to further reduce the cost of cloud detection
% \end{packeditemize}



% \jc{there can be a nice 1-on-1 mapping between the key questions and challenges:
% \begin{itemize}
%     \item how to pick a good ref image? => challenging because the latest images may not be the best choice, as they can be cloudy.
%     \item how to do change detection? => challenging because one needs to detect cloud and lumination shift despite limited on-board compute.
%     \item how to select the best configuration? => challenging because (1) a large config space, and (2) badly compressed images affect future compression.
% \end{itemize}}


% Answering these questions is not trivial, because
% \begin{enumerate}
% \item The state-of-the-art algorithms that can detect changes under varying cloud and illumination conditions are too compute-intensive (neural network with ?? layers) for the satellite to afford.
% Need to design cheap algorithms that can accurately detect changes under limited satellite computation.
% \item It is difficult to select the configuration that configures the system in a way that can cope with various resource constraints while maximally improving the image quality of the downloaded images, since there are a lot of configurations to choose and the configurations vary between different locations.
% \item How to obtain up-to-date cloud-free images as the reference images for those locations that can be cloudy for a long time?
% \end{enumerate}

% \begin{packeditemize}
% \item \textbf{Lower storage requirement on the satellite}: The reference images of an area can be stored on the ground and only need to be uploaded to the satellite right before visiting that area.
% As a result, the satellite only needs to be stored on the ground.
% \item \textbf{Higher compression potential}: we can achieve higher potential by using rich computation on the ground and using images from different satellites as the reference. 3 concrete potentials:
% \begin{packedenumerate}
%     \item The ground can pick a more up-to-date reference image by using images from other satellites. \kt{Need to quantify the potential}
%     \item The ground can customize the compression configuration for different locations. \kt{Need to quantify the potential}
%     \item \kt{Another benefit: stitching multiple images together, enabling us to get a cloud-free image even for locations that are always cloudy. I guess it is a bit early to bring this point here so I put it in the comments}
% \end{packedenumerate}
% \end{packeditemize}
% The reference images only need to be stored for several hours
% satellite frequently visits the ground, each visit has uplink,
% satellite only need to store images between two consecutive visits
% only tens of locations will be visited between two uplinks.
% As the satellite 
% This allows the satellite to only cache XXX \kt{a concrete number here} reference images 
% As the satellite 
% is available, the satellite can \textbf{discard} historical images cached for previous locations and receive historical images for future locations from the uplink.
% \item New trend: there is much more uplink capacity than before when the satellite contacts the ground station.
% Thus, when the uplink is available, the satellite can \textbf{discard} previous cached historical images and cache new historical images from the uplink.
% \kt{This sentence is difficult to write, discuss}
% only needs to store historical images before the next contact with the earth, allowing the satellite to store historical images for a small subset of locations that the satellite visits.
% During each contact, we can stream historical images for the locations that the satellite will pass before next location.
% The satellite thus does not need to store historical images for locations  needs to keep historical images for \textit{locations} before the next contact to the ground station. 
% \item 1st contribution: measurement study that shows {\em if} each satellite has access to ALL history images (in their perfect quality) from ALL satellites, xxx\% fewer regions need to be compressed than without history images. \jc{THIS IS THE 1ST KEY RESULT}
% We present \name, the first system that improves on-board satellite imagery compression leveraging change-based encoding.


To test the end-to-end performance and resource usage, we design and implement a detailed prototype of \name, including the algorithms for change detection, cloud detection, and illumination alignment (\S\ref{sec:dynamism}).
We evaluate \name using realistic satellite specifications (including uplink, downlink, and storage capacities) of the DOVEs satellite constellation.
We test \name on two datasets: one with \fillme~TB data collected from Sentinal-2 covering an area of \fillme million km$^2$, and the other with \fillme~TB data collected from Planet (including 6 satellites) covering an area of \fillme million km$^2$.
Our evaluation shows that \name can reduce the downlink demand by up-to 50\% (and up-to \fillme\% during summer time) without hurting the image quality compared to the best baseline.
Moreover, \name achieves these improvements without exceeding the uplink capacity and on-board storage limit. 
% sticks within the limited uplink bandwidth and does not impose extra storage overhead on the satellite.
% \jc{need more concrete numbers}
% images of xxx\% more earth surface every xxx hours at a xxx\% higher quality than the smartest baseline. \kt{also highlight other eval results}


% That said, \name has its limitations. For example, \name compresses the images in a \textit{lossy} manner, which may not be ideal in applications that require ultra-high fidelity (\eg military applications). Please refer to \S\ref{sec:limitation} for a full set of limitations.
% :
% \begin{itemize}
%     % \item We test our system based on Level 1C satellite data, which are not the raw sensed data from the satellite, but instead the data after noise removal and image alignment. However, the performance gain should remain similar
%     \item First, \name 
%     \item Second, \name compresses the images in a \textit{lossy} manner. However, we argue that lossy images are suffice for a wide range of applications. \kt{Need more arguments on this point.}
% \end{itemize}


==> tex-files/intro.tex <==
%!TEX root = ../paper.tex
%!TEX spellcheck = en_US


\section{Introduction}


% Satellite imagery, and its corresponding applications, are growing rapidly.
High-quality satellite imagery is key to a wide range of applications. 
With more satellites capturing more images at higher resolutions, satellite imagery has promised to transform
% The increased availability of satellite images with high resolution and short revisit time have enabled 
numerous applications in digital agriculture ~\cite{mulla2013twenty, hank2019spaceborne,planet-digital-agriculture,digital-agriculture1}, environmental monitoring~\cite{manfreda2018use, tucker2000strategies, tralli2005satellite, cunjian2001extracting,environment-monitoring1}, automatic road detection~\cite{kopsiaftis2015vehicle, van2018spacenet,automatic-road-detection} and many more.
% However, limited by the downlink capacity, the satellite imagery captured by the satellite cannot be fully downloaded by the satellite.
However, the reality is that most satellite imagery data are not received on the ground due to {\em limited downlink capacity}.
% However, bottlenecked by the downlink capacity, 
By one estimate, only 2\% of the total images observed by the satellite can be downloaded to the ground~\cite{kodan}.\kt{TODO: add citations here}
%Despite efforts to expand the downlink capacity, they incur high costs to deploy more ground stations and reserve more bandwidth.
%As a result, downlink capacity remains a bottleneck, which severely limits the coverage, fidelity, and freshness of images available to applications.


%Different satellite constellations tackle this downlink bottleneck differently.
%% depending on their missions. 
%%Facing this downlink bottleneck, there are two types of satellite \textit{constellations} that handle this bottleneck in different ways.
%% \peder{the ground can download?}
%Mission-based satellite constellations~\cite{kodan,oec} focus on a small fraction of 
%%The first type of satellite constellations~\cite{kodan,oec} are built with a mission that focuses on a small subset of 
%geographical locations that are pre-determined by certain applications. 

Many previous efforts tackle this downlink bottleneck in the context of mission-based satellite constellations~\cite{kodan,oec}, focus on a small fraction of geographical locations that are pre-determined by certain applications. 
For instance, Biomass mission~\cite{biomass} targets forest areas.
These satellites run mission-specific filters (\eg forest filter for Biomass mission~\cite{??}), so the images of the selected areas can be downloaded with existing downlink capacity.
%As a result, these satellites run mission-specific filters (\eg forest filter for Biomass mission) to filter out a large percentage of the areas on the earth (\eg about 91\% earth surfaces can be filtered out~\cite{forest-area,ocean-area} using forest filter), so the downlink capacity is sufficient for downloading the data of remaining areas.
However, these mission-based satellites may filter out data useful for other applications.
For instance, a forest filter will filter out about 91\% earth surfaces~\cite{forest-area,ocean-area}, including agricultural areas, which can be crucial for crop monitoring applications.

Rather than improving the filtering on mission-based satellites, the focus of this work is to enable better on-board image compression for general-purpose satellites, such as Sentinel-2~\cite{sentinel-2}, PlanetScope~\cite{planet}, Landsat~\cite{landsat}, which aim to download all earth imagery data with high coverage, freshness and fidelity.\footnote{We want to clarify that this work is orthogonal to the recent proposals to improve the low-earth orbital (LEO) satellite constellations that are designed for Internet connections, such as Starlink.}
%Many satellite constellations (\eg Sentinel-2~\cite{sentinel-2}, PlanetScope~\cite{planet}, Landsat~\cite{landsat}) are general-purpose and aim to download all earth imagery data.
Unfortunately, today these satellites have to compress the imagery data aggressively at the cost of either fidelity or freshness of the downloaded images. 
%%The second type of satellite constellations are designed with a general-purpose mission that instead aims to download data all over the earth (\eg Sentinel-2~\cite{sentinel-2}, PlanetScope~\cite{planet}, Landsat~\cite{landsat}).
%This type of satellites handle the downlink bottleneck in two ways. 
%% either by downloading low-resolution satellite imagery or augmenting the downlink capacity (\eg Sentinel-2, PlanetScope).
%% Both choices are not ideal.
%The first way is to download low-resolution satellite imageries.
For example, MODIS constellation~\cite{MODIS} downloads imageries with a ground sample distance (defined as the distance between the center of pixels, GSD for short) of 250m.
However, such low-resolution images do not suffice for applications like crop growth monitoring and urban expansion analysis (which requires a GSD of 5-30m~\cite{application-GSD}), or applications like 3D city monitoring and precision agriculture, (which require a GSD of 1-5m~\cite{application-GSD}).
Alternatively, satellite imagery providers may expand the downlink capacity by building more ground stations or parallelizing the download across satellites in a constellation~\cite{planet,sentinel-2,kodan}.
However, despite these efforts, a large fraction of images (\textit{e.g.} ocean areas in Sentinel-2~\cite{sentinel-2}) still cannot be downloaded.

%\jc{i removed the cost argument agains expanding capacity because it's been discussed in the 2nd paragraph. Kuntai, please move the text there if you see appropriate.}
% \jc{The cost argument seems to be misplaced here: with their current DL capacity, is Sentinel-2 or PlanetScope already capable of downloading everything at a desirable quality level? If they already do, then why bother? If they have already deployed enough capacity, saving the cost for them seems like weaker position. But I guess even with the new DL capacity, the bottleneck still remains (which is a stronger position), right? If so, let's don't put the cost argument here.}
% \jc{Sending more satellites increases the DL capacity? Thßis seems counterintuitive. Won't having more satellites produce more images instead?}

%Rather than improving the filtering on mission-based satellites, the focus of this work is to enable better on-board image compression for general-purpose satellites to download more images at better fidelity under limited downlink capacity.\footnote{We want to clarify that this work is orthogonal to the recent proposals to improve the low-earth orbital (LEO) satellite constellations that are designed for Internet connections, such as Starlink.}


%The research focus of this paper, is to handle the downlink bottleneck of general-purpose satellite constellations by improving the on-board satellite image compression, so that existing general-purpose satellites can download more images to the ground station, and future general-purpose satellite constellations can be built and maintained with less cost.


\jc{the next 5-6 paragraphs need to be tightened}

There has been an active research on satellite imagery compression (\eg~\cite{satroi,virtual-background,change-encoding}).
A basic observation behind it is that 
%Prior work~\cite{satroi,virtual-background,change-encoding} identifies an opportunity to further compress satellite imagery: 
the geographical content is mostly unchanged between two consecutive satellite visits.
This observation inspires \textit{change-based encoding}:
one can use a previous image from prior satellite visits at the same terrestrial location as the reference to identify the changed regions in the current satellite visit and focus the encoding only on the changed regions.
%We call this approach \textit{change-based encoding.}
Using such change-based encoding, the satellite only needs to download ??\% of the geographical areas in average, a ??x compression (see \S\ref{??} for the details of our measurement).\peder{Missing numbers here...}
% \item
% First type of work: existing satellite imagery encoders. Cons: areas that are not changed also need to be downloaded. \kt{Merge para 3.}

Though promising, such change-based encoding heavily relies on \textit{up-to-date, cloud-free} reference images as reference. %in order to significantly save the usage of downlink.
For instance, in an agriculture application, if the reference image is (partly) covered by clouds,  then it will be impossible to determine if some changes have occurred to the pixels of the current image that overlap with the clouds, and as result the satellites may encode and send more pixels than necessary.
Similarly, if the reference image is out-of-date, more pixels will be sent than necessary because  other satellites may have captured and transmitted the same content recently.

\jc{two key ideas: (1) use more satellites to get up-to-date cloud free, (2) how to best leverage uplinks}

%For example, in agriculture areas, the color of the soil changes significantly after raining.
%Thus, all soil areas will be counted as change and be downloaded if we use a reference image before the rain happens.
%Empirically, we measure the amount of changes with respect to the staleness of the reference image, and found that XXX.



As a result, the challenge of implementing such change-based encoding is \textit{how to obtain fresh, cloud-free reference images on-board}.
Prior work~\cite{satroi,virtual-background,change-encoding} stores the reference image on-board (with sufficient compression to fit into on-board storage) and update the reference images when a new cloud-free image is observed.
However, the reference image of this approach is stale due to two reasons.
First, as the satellite revisits the same location once every 10 days~\cite{sentinel-2-revisit}, the satellite can only refresh the reference image for that location once every 10 days.
Second, when a new image is observed, that image can be cloudy and cannot be used as future reference, thus further postpone the updating of the reference image.
% Facing this design question, prior work~\cite{satroi,virtual-background} uses the on-board storage to store the reference images for all geographical locations are stored on the satellite.
% However, to store reference images for all locations, the reference images need to be aggressively compressed with a compression rate larger than 400, which forces the satellite to download more than half of the areas in order to cover all the changes (see detailed measurements in \S\ref{??}).\peder{missing reference}



% First, the satellite does not have sufficient on-board computing power to handle the dynamics above the ground, like clouds and shadows. 
% Even though these areas can be efficiently skipped, 
% Second, the satellite does not have sufficient storage to store a reference image for every area that the satellite visits, as this requires storing ??PB of the data on the satellite, ??x larger than the satellite disk capacity even after compressing the images by ???x.
% \kt{Give people a sense of how expensive it is to expand the on-satellite storage.}
% Even if the satellite \textit{could} have a disk with almost infinite storage that can save the latest historical images of all regions, XXX.

% \kt{Need to confirm with Peder why the satellites cannot have disks with super large capacity} \jc{while you check with peder, can we claim something like ``even if a satellite does store the latest history images of all regions and uses them to detect only changes, its still not efficient since the more recent the ref image is the better, and each region is photoed by the same satellite only once every xxx days but will be by {\em some} satellite every xxx hours?''}

% \kt{I am thinking of also mentioning the reason that the satellite does not have enough compute to handle clouds. Pros: }
% \item 
% \kt{New reality: uplink, on-board computing}
% \kt{New reality inspires a new pipeline}
% \kt{Realize this potential, key design questions (reference image, configuration, cloud/illumination}
% \kt{Why answering these questions are not trivial?}

% We observe a new trend on the satellite: the \textit{on-board computing} on the satellite becomes more abundant, and the \textit{uplink capacity} from the ground station to the satellite is becoming larger and larger.
% For example, \kt{a list of data to instantiate this point.}

% \jc{we should emphasize that the ref image can be from {\em any} satellite that has flown by the location recently} 
% \jc{we should highlight that our design enables each satellite to virtually have access to images taken by {\em all} satellites to compress each image.}
% To store reference images under limited on-board storage, our insight is that: for a given geographical location, its corresponding reference image only needs to be on-board when the satellite flies by that location.
% In other word, instead of saving the reference images for all locations, the satellite only need to save the reference images for \textit{a small subset} of locations that the satellite is going to fly by.

% Based on this insight, we advocate for a design that the ground upload the reference image to the satellite for the locations that the satellite will visit before next ground contact.
We advocate for a new design that leverages the \textit{uplink} to update the reference images on the satellite.
By leveraging the uplink, this design allows the satellite to refer to images \textit{from the whole satellite constellation}, which significantly improves the freshness of the reference images.
As a result, the satellite can obtain more \textit{up-to-date} cloud-free reference images.
Concretely, for DOVEs constellation~\cite{planet}, if one location is cloud-free, our design allows the satellite to update its reference image \textit{daily}, 10x more frequent than updating the reference images by the satellite itself.
% (the link from the ground to the satellite) to update the reference images on the satellite, so that each reference image only needs to be on-board  the storage demand on the satellite. Concretely, we let the satellite cache the reference images for \textit{a small subset} of locations, and \textit{timely update} this cache to make sure the satellite have access to future locations.
% \kt{A figure to contrast prior design and our design}
% Then, the satellite captures the image for that location, compares this image with the reference image, and only stores the changed areas.
% Then the satellite captures the image of this location, saves the parts that differ from the reference image, and deletes the reference images after use. 
% Compared to prior design that stores reference images for all geographical locations, the advantage of our design is two-fold:
% \begin{packeditemize}
%     \item Our design enables the satellite to use the images from \textit{other satellites} as the reference.
%     access higher-quality reference images\kt{quantify}, which allows the satellite to download only 10\% areas while still covering all changes.
%     \item Further, this design allows the satellite to access a more up-to-date reference image by using the images from \textit{other satellites} as the reference. 
%     To show the concrete potential, we perform a measurement in \S\ref{??} \kt{fill in more details here}
% \end{packeditemize}


% First, this design increases the potential of change-based encoding. By streaming the reference image up to the satellite, the satellite can access images from \textit{other satellites}, enabling it to stream a more up-to-date reference image to the satellite.
% First, this design allows the ground to streaming the images from \textit{other satellites} as the reference. The satellite can thus obtain a more up-to-date reference image and download much fewer changed areas compared to using the images from the satellite itself as the reference image.
% df downloaded while still maintaining  obtain a more up-to-date reference image, thus the satellite can encode much less areas 
% uploading the reference images from the ground, the satellite virtually has access to the images taken by \textit{all} satellites, which provides much higher compression capability than ABC.

% Second, this design significantly reduces the resource demand of performing change-based encoding on the satellite, in terms of both storage and on-board computing power.
% This is because the satellite can immediately delete the reference image of one location after it finishes visiting that location.
% This reduces the number of reference images that the satellite needs to store from ??? to ???, a ???x reduction.
% Also, the ground can customize the cloud detector and the change detector based on different geographical locations and other satellites. As a result, the satellite can perform accurate cloud detection using a cheap decision-tree-based cloud detector (rather than an expensive neural-network-based cloud detector~\cite{??}).
% Second, this design reduces the storage requirements on the satellite by ????x compared to storing all reference images on the satellite, making it possible to fully leverage the potential of only downloading changed areas under limited satellite storage space.


% \jc{i'd seriously downplay the first question. it's more like an ml question. i understand you spent a lot of time on it, and it's important to make it work, but it's not really relevant to "how to leverage the big pool of history images", which is the key up until this point in the story}
% \jc{this sounds more like why (3) is challenging, not a design question..}
% \jc{i'd put this upfront. this is the key challenge.}
% To realize this potential, we list three design questions are:
% \begin{enumerate}
%     \item How to detect changes on the satellite, given the varying cloud and illumination conditions? 
%     \item How to obtain the best image quality (in terms of PSNR) under limited satellite computation power, storage, and limited link capacity between the satellite and the ground station?
%     \item How to develop a mechanism to avoid letting the error (introduced by not downloading some of the areas) propagate. 
%     \item How to select reference images? 
% \end{enumerate}


To instantiate the design above, we propose \name, the first system that improves satellite imagery compression by leveraging historical earth observations. 


\begin{figure}
    \includegraphics*[width=1\columnwidth]{figures/earth-satellite.jpg}
    \caption{\name uploads the reference images for a small subset of future locations, which the satellite will fly-by before next ground contact.}
    \label{fig:uplink-design}
\end{figure}


% The major practical challenge of \name is that the total file size of reference images significantly exceeds the limited uplink capacity (only 250kbps~\cite{dove-uplink-downlink} for DOVEs constellation) of earth observation satellites.
% To handle the limited uplink, \name stores the reference images on-board and update a small subset of reference images (where the satellite will fly-by before next ground contact) during each ground contact.
% We illustrate this design in Figure~\ref{fig:uplink-design}.


% Compared to prior solutions that encode and download observed images in their entirety, \name stores the reference images on-board without requiring more on-board storage due to the following two reasons:
% \begin{packeditemize}
%     \item Compared to current satellites that stores every pixel of the captured images on-board, \name only saves changed pixels on-board, squeezing out limited storage space for \name to store reference images.
%     \item Even though the reference images need to be heavily compressed to fit into this limited storage space, the changes can still be accurately detected and downloaded (with marginal cost of slightly downloading more areas than necessary --- we will quantify this overhead in \S XX).
% \end{packeditemize}

% Besides the compression of the reference images, \name further cut down the usage of uplink using the following two optimizations:
% \begin{packeditemize}
%     \item During each ground contact, the ground only need to update references for those locations that the satellite will fly-by before the next ground contact, which is $160\times$ smaller than the total number of locations.
%     \item  The ground only needs to upload the \textit{difference} between the on-board reference images and the reference images to be uploaded. This can significantly reduce the amount of data need to be transferred, as the reference images to be uploaded are the same as the on-board reference images on most of the geographical areas.
% \end{packeditemize}
% With these two optimizations, \name is able to update the corresponding reference image before capturing a new image.

A primary challenge with \name is the substantial file size of reference images, which surpasses the limited uplink capacity (250kbps\cite{dove-uplink-downlink} for the DOVEs constellation) of earth observation satellites. To address this, \name retains reference images on-board and updates a subset corresponding to imminent trajectory of the satellite during each ground contact. This approach is depicted in Figure~\ref{fig:uplink-design}.

Unlike traditional methods that download observed images in their entirety, \name stores reference images without requiring additional storage space. This is achieved by:
\begin{packeditemize}
\item Only saving the pixels that have changed, thus conserving space that can be allocated for reference images.
\item Compressing the reference images to fit within the storage constraints. Despite this compression, \name is capable of detecting and downloading over 99% of the changes. However, there's a trade-off: occasionally, areas slightly larger than necessary are downloaded. This overhead is elaborated upon in \S XX.
\end{packeditemize}


In addition to compressing reference images, \name further optimizes uplink usage in two ways:
\begin{packeditemize}
\item During each ground contact, only references for imminent satellite trajectories are updated, reducing the locations updated by a factor of $160\times$.
\item Only the \textit{difference} between on-board and new reference images is uploaded, reducing data transfer as most images remain largely unchanged from their previous upload.
\end{packeditemize}
These strategies enable \name to refresh the relevant reference image prior to a new capture.

% To handle such limited uplink, \name amortize the uploading of the reference images across different ground contacts.
% Concretely, during each ground contact, \name uploads the reference images for a small subset of future locations, which the satellite will fly-by before next ground contact. \jc{Doesn't this mean reference images will be less up-to-date? It seems to defeat the previous claim that reference must be up-to-date, right?}
% Further, \name only streams the difference between the reference images to be  uploaded and the reference images on-board.
% With these two optimizations, \name is able to provide a new reference image everytime when the satellite captures a new image, without exceeding limited uplink bandwidth.

% \jc{I think it's necessary to bring up the insight that low-quality reference is enough for change-based encoding. Otherwise, because you need a reference in each location, the storage cost will be prohibitive.}



% \begin{packedenumerate}    
%     \item 
%     How to upload the reference images to the satellite, given the extremely limited uplink capacity (only 250kbps~\cite{dove-uplink-downlink})?
%     % \item 
%     % How to determine the policy of uploading reference images (\ie which locations should have their reference images uploaded in what quality), in a way that is aware of the varying uplink capacity (characterized in \S\ref{??}), while still allowing the satellite to access high-quality reference image?
%     \item 
%     How to detect changes under varying cloud condition (and also illumination condition) so that almost all changes can be detected without exceeding the computation capacity on-board?
% \end{packedenumerate}


% To upload reference images under limited uplink, \name only updates the difference between the reference images to be uploaded and the current reference images on-board.
% This significantly saves the am


Another challenge of \name is to detect changes while fitting into the limited computation resource on the satellite.
The change detection process is computationally expensive as it needs to  detect changes under varying cloud coverage condition, while accurately identifying clouds require running tens of layers of neural networks~\cite{change-encoding,cloud-net}.
To reduce the computation cost of change detection process, our insight is that cheap algorithms (\textit{e.g.} decision-tree-based cloud detector and pixel-difference-based change detector) can already accurately predict changes on over XX\% of the geographical areas.
% \jc{what does this cheap algorithm have to do with the use of uplinks?}
As a result, \name runs cheap algorithms to detect changes, and download the changes together with the areas that the cheap algorithms are likely to produce errors.




% We proposes three techniques to address these challenges. \kt{need to fill the detail of these techniques}.
% \begin{packeditemize}
%     \item Obtaining the reference image $\rightarrow$ reference image stitching
%     \item Varying uplink condition $\rightarrow$ keep more images on the satellites to safeguard against potential ground disconnection
%     \item Change detection using limited resource $\rightarrow$ 1. perform coarse-grained cloud and change detection, using cheap algorithm. Insight: cheap algorithm may perform really bad in its application-specific metric, 2. using reference image to further reduce the cost of cloud detection
% \end{packeditemize}



% \jc{there can be a nice 1-on-1 mapping between the key questions and challenges:
% \begin{itemize}
%     \item how to pick a good ref image? => challenging because the latest images may not be the best choice, as they can be cloudy.
%     \item how to do change detection? => challenging because one needs to detect cloud and lumination shift despite limited on-board compute.
%     \item how to select the best configuration? => challenging because (1) a large config space, and (2) badly compressed images affect future compression.
% \end{itemize}}


% Answering these questions is not trivial, because
% \begin{enumerate}
% \item The state-of-the-art algorithms that can detect changes under varying cloud and illumination conditions are too compute-intensive (neural network with ?? layers) for the satellite to afford.
% Need to design cheap algorithms that can accurately detect changes under limited satellite computation.
% \item It is difficult to select the configuration that configures the system in a way that can cope with various resource constraints while maximally improving the image quality of the downloaded images, since there are a lot of configurations to choose and the configurations vary between different locations.
% \item How to obtain up-to-date cloud-free images as the reference images for those locations that can be cloudy for a long time?
% \end{enumerate}

% \begin{packeditemize}
% \item \textbf{Lower storage requirement on the satellite}: The reference images of an area can be stored on the ground and only need to be uploaded to the satellite right before visiting that area.
% As a result, the satellite only needs to be stored on the ground.
% \item \textbf{Higher compression potential}: we can achieve higher potential by using rich computation on the ground and using images from different satellites as the reference. 3 concrete potentials:
% \begin{packedenumerate}
%     \item The ground can pick a more up-to-date reference image by using images from other satellites. \kt{Need to quantify the potential}
%     \item The ground can customize the compression configuration for different locations. \kt{Need to quantify the potential}
%     \item \kt{Another benefit: stitching multiple images together, enabling us to get a cloud-free image even for locations that are always cloudy. I guess it is a bit early to bring this point here so I put it in the comments}
% \end{packedenumerate}
% \end{packeditemize}
% The reference images only need to be stored for several hours
% satellite frequently visits the ground, each visit has uplink,
% satellite only need to store images between two consecutive visits
% only tens of locations will be visited between two uplinks.
% As the satellite 
% This allows the satellite to only cache XXX \kt{a concrete number here} reference images 
% As the satellite 
% is available, the satellite can \textbf{discard} historical images cached for previous locations and receive historical images for future locations from the uplink.
% \item New trend: there is much more uplink capacity than before when the satellite contacts the ground station.
% Thus, when the uplink is available, the satellite can \textbf{discard} previous cached historical images and cache new historical images from the uplink.
% \kt{This sentence is difficult to write, discuss}
% only needs to store historical images before the next contact with the earth, allowing the satellite to store historical images for a small subset of locations that the satellite visits.
% During each contact, we can stream historical images for the locations that the satellite will pass before next location.
% The satellite thus does not need to store historical images for locations  needs to keep historical images for \textit{locations} before the next contact to the ground station. 
% \item 1st contribution: measurement study that shows {\em if} each satellite has access to ALL history images (in their perfect quality) from ALL satellites, xxx\% fewer regions need to be compressed than without history images. \jc{THIS IS THE 1ST KEY RESULT}
% We present \name, the first system that improves on-board satellite imagery compression leveraging change-based encoding.

Our evaluation shows that \name can gather images of xxx\% more earth surface every xxx hours at a xxx\% higher quality than the smartest baseline. \kt{also highlight other eval results}



That said, \name has two limitations:
\begin{itemize}
    % \item We test our system based on Level 1C satellite data, which are not the raw sensed data from the satellite, but instead the data after noise removal and image alignment. However, the performance gain should remain similar
    \item First, \name requires a high uplink capacity from the ground station to the satellite, which does not apply to all satellites.
    \item Second, \name compresses the images in a \textit{lossy} manner. However, we argue that lossy images are suffice for a wide range of applications. \kt{Need more arguments on this point.}
\end{itemize}

\peder{There are too many bullet points - to the point where it's hard to follow: Can we shorten this to: \name requires a high uplink capacity and compresses images in a \textit{lossy} manner.  While this suffices for a wide range of application, this is not done for most satellite constellations.  } 


==> tex-files/intro_old.tex <==
\section{Introduction}
\label{sec:intro}

Rough outline of the story:
\begin{itemize}
    \item LEO satellites are growing, becoming more popular, and large in size
    \item the main challenge is the limited and intermittent downlink to the ground. observed data $>$ downlink data
    \item OEC (orbital edge computing) has been proposed, to process data in space, send only important data, and reduce downlink gap. This has become feasible with the new trend of placing more and COTS (commodity of the shelf) compute on the satellite.
    \item smart compression of satellite images, seems like a natural choice to reduce this DL bottleneck
    \item the topic of compression has been studied, with simplistic approaches built for specialized and very limited HW traditionally on satellites [cite, JPEG 2000, etc].
    \item some work has looked at using the emerging large compute capacity of OEC for compression, using auto encoders[cite]. 
    \item but both these approaches are context agnostic, and treat all images similarly. 
    \item we observe a unique feature of satellite imagery-- images rarely change (add chart and numbers). 
    \item this feature is what has been used on other works, processing on the earth, by only storing diffs in images, rather than full images [cite].
    \item in this work, we propose \name{}, that leverages the insight from historical imagery, alongside the emerging compute capacity in OEC, as a first system that does diff-based compression in space.
    \item \textbf{Challenges}
    \begin{enumerate}
        \item \textit{access to historical images in space:} one of the main barriers to diff based approaches is that you need to compare against a historical reference. While on the earth, there are large datastores with months, or even years, of historical images, captured by multiple satellites, this rich dataset is not available in space. 
        \item relying on just captured images by the satellite is not sufficient. \shadi{how to show this? any argument, numbers? }
        \item streaming to satellites is even harder, with uplinks being an order of magnitude smaller than downlink.
        \item \textit{dynamism of the images:} satellites trajectories are predictable, but still lots of dynamism. the two biggest are 1) clouds 2) illumination. these need pre-processing before compression is feasible. One of the main barriers to doing diff-based compression in the past on the satellites.
        \item \textit{limited resources:} limited uplink, downlink, storage, and compute [add numbers and citations]. 
        \item satellites move and constantly capture new areas. revisit rates can large, e.g., X. 1) having reference images for all areas quickly becomes a large amount of storage. 2) uploading all this data becomes prohibitive. 3) processing all images becomes compute-intensive. \shadi{numbers to support this?}
    \end{enumerate}
    \item \name overcomes these challenges by smartly using the limited resources in a way that does not impact the quality of compressed images compared to state-of-the-art approaches.

    \item \textbf{Contributions:}\shadi{I found enumerating this a bit challenging. what are our main contributions \& novelties?}
    \begin{enumerate}
        \item analysis of feasibility and value of compression in space
        \item exhibiting the possibility of compressing satellite imagery with high quality when using highly down-sampled reference images and analyzing the trade-off space.
        \item smart utilization of limited compute resources in space by using a mix of a) context-aware specialized models, b) \shadi{dynamic?} resolution reduction of captured images to be processed, c) conservative labeling of areas to be downloaded.
        \item \shadi{maybe something along the lines of:} smart replacement strategy to a) reconstruct new historical reference from a constellation of satellites on earth and b) upload a historical reference to the satellites.
    \end{enumerate}
\end{itemize}

==> tex-files/outline.tex <==




\begin{outline}
\1 Satellite imagery is popular.
\1 Downlink insufficient
\1 Two types of satellite systems:
    \2 System 1: 
    \2 Application 2: satellite
\1 Our goal: alleviate the downlink bottleneck of ground satellite using compression.
\1 Prior approach: change-based encoding
\1 Not applicable: limited on-board storage, change-based encoding not applicable.
\1 We advocate for uplink-based approach.
\1 Design benefit:
    \2 Reduce the storage cost
    \2 Allow accessing latest reference from other satellites
    \2 Allow better cloud detection
\1 Satellite-side challenge:
\2 How to detect change under varying cloud and illumination conditions
\2 How to fit into the resource budget on the satellite.
\1 Ground-side challenge:
\2 How to get the latest reference image
\2 How to handle varying uplink conditions?
\1 2. How to detect the changes after having the reference image on-board?
\2 A natural solution is to leverage techniques in video encoding literature to detect changes.
However, video encoding assumes that the difference between two consecutive frames is minor, which is not true for satellite imagery as the illumination condition and cloud condition can vary a lot.
\2 Current change-based encoding for satellite imagery is not applicable on the satellite as it requires both high-quality reference image and is computationally expensive.
\1 Satellite-side technique
\2 Handle cloud and illumination conditions using the following workflow:
    \3 Cloud detection and removal (assuming the cloud data can be discarded)
    \3 Illumination alignment (we use a simple linear regression algorithm to determine the lighting change).
    \3 Change detection
    \3 Encode and store the changes
\2 Reducing storage cost
    \3 Downsample the image by 16x, width and hight
    \3 We found that it can still detect 99\% of the changes.
\2 Reducing computation cost
    \3 Detecting cloud requires much less computation cost if there is a reference image
\2 Safeguarding mechanism
    \3 When in doubt of whether an area is changed/cloudy, download
    \3 Guarantee downloading an area once every 2 months
\1 Ground-side technique
    \2 Obtaining latest reference images
        \3 Challenging: latest image may be cloudy
        \3 Solution: stitching multiple images
    \2 Handing varying uplink bandwidth
        \3 Charactering the uplink
        \3 Solution: let the satellite store more images (to handle disconnection) with less image quality (to handle limited bandwidth)


\end{outline}

\kt{Discuss: why prior work does not upload reference image on the satellite}
\kt{Discuss: Uplink of earth observing satellite seems to be limited.}
\newpage




==> tex-files/technical.tex <==

- Section 2: reference image stalenesss correlates with change detection

\section{\name: update reference via uplink}


- we use uplink to reduce the reference image staleness

- workflow: upload reference -> detect change -> download change

- key challenge: how to use limited uplink capacity to update reference

- insight: 
1). low-resolution reference image can detect changes compared to low-qp image. 
%2). only update reference images when cloud-free
3). Periodical reference image update. Strawmen: update reference everytime when downloading a new change. Not good: some block maybe updated multiple times between two consecutive satellite visit



\section{Updating reference using uplink}

- Start with a hypothetical baseline ==> no uplink, local, change detection, per-block update
- Idealized global view baseline ==> per-block update using multiple satellite update
- Need a trade-off figure, uplink <---> downlink
- Disadvantage: high uplink usage.
    - Idea 1: reference image compression. low-resolution reference image can detect changes compared to low-qp image. 
    - Idea 2: Batched reference image update. Strawmen: update reference everytime when downloading a new change. Not good: some blocks maybe updated multiple times between two consecutive satellite visits
- Safe-guarding 



\section{\name: update reference via uplink}



\subsection{Uplink-based design}

\begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.99\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/contrast-no-uplink.pdf}
         \caption{Updating reference images with local images on the satellite. }
         \label{fig:uplink-design:no-uplink}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.99\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/contrast-with-uplink.pdf}
         \caption{Updating reference images via uplink.}
         \label{fig:uplink-design:with-uplink}
     \end{subfigure}
     \caption{Contrasting two reference image uploading policies: (a) using local images captured by the satellite itself and (b) uploading images using uplink. By uploading images using uplink, one can reduce the time gap between reference images and captured images (\ie the staleness) from 15 days on average to 5 days on average.}
     \label{fig:uplink-design}
\end{figure}



% \kt{Should I put this into a single section or merge with prior section? I feel like typically section 3 is an overview, but I want to highlight the uplink-based design (instead of burying it inside section 2}
% \kt{The goal of this section is to demonstrate the benefit of using uplink without diving into concrete system components and challenges.}


% \subsection{Improving reference images via uplink}


\jc{some background is missing here: what is an uplink? what is it usually used for? what is a "ground contact"? maybe put background basics like them before 2.1, and remind people at the beginning of sec 3?}


We advocate that the satellite constellations can use uplink to greatly reduce the staleness of reference images.
This is because the uplink allows the satellite to receive and use images \textit{from any satellite in the same constellation} as the reference images, while the satellite can only use images from itself as the reference without the uplink.
% \begin{packeditemize}
% \item During ground contact, images for upcoming fly-by locations before the next ground contact are uploaded to the satellite.
% \item When passing over a location, the satellite captures and encodes changes using the corresponding reference image.
% \item During the next ground contact, the ground downloads the changes from the satellite.
% \end{packeditemize}.
To further illustrate how much uplink could reduce the staleness of reference images, we provide an illustrative example and a measurement.

% We advocate for an \textit{uplink-based} design: instead of letting the satellite store and update reference images, we let the ground upload the reference images to the satellite.
% We visualize this design in Figure~\ref{fig:uplink-design}. Concretely,
% \begin{packeditemize}
%     \item When contacting the ground: the ground uploads reference images for all locations fly-by before the next ground contact.
%     \item When flying by a geographical location: the satellite captures the image for that geographical location, then calculate and encode the changes using the reference image for that location
% \end{packeditemize}


% \begin{packeditemize}
%     \item During current ground contact: the ground upload reference images for locations before next ground contact.
%     \item Before next ground contact: the satellite photos the earth and only encode the changes
%     \item During next ground contact: the satellite send the encoded changes to the ground.
% \end{packeditemize}
% We visualize this design in Figure~\ref{fig:uplink-design}

% \begin{figure}
%     \includegraphics*[width=1\columnwidth]{figures/earth-satellite.jpg}
%     \label{fig:uplink-design}
% \end{figure}

% Compared to storing the images by the satellite itself, our \textit{uplink-based} design allows the satellite to:
% \begin{packeditemize}
%     \item \textit{Store less-compressed reference under limited storage.}
%     By uploading the reference images to the satellite, the satellite only needs to store the reference images for \textit{a small subset of geographical locations} that the satellite will fly by before the next ground contact.
%     \item \textit{Use latest reference images from other satellites}
%     By uploading the reference images to the satellite, the satellite can refer to the latest reference image that may come from other satellites.
% \end{packeditemize}

% To measure the effect of such \textit{uplink-based design} on reference images, we perform an idealized measurement using the specification of a satellite from DOVEs constellation (with 720GB storage space) as an example.
% \kt{need to search and write more setups here}
% We assume the uplink is available at every ground contact with sufficient bandwidth (we will discuss and handle the real uplink condition in \S\ref{??}).
% We show that
% \begin{packeditemize}
%     \item The reference image only needs to be compressed for 20x, while the reference images need to be compressed for 500x if reference images are stored and updated by the satellite itself.
%     \item For a given location, the satellite can use images older than 90 minutes as the reference image. In contrast, the satellite can only use images older than 10 days as the reference (as the satellite.
% \end{packeditemize}


\mypara{Example on how uplink reduces staleness}
By leveraging the uplink, our design enables the satellite to obtain images from \textbf{\textit{other}} satellites.
This can significantly reduce the staleness of the reference image. We illustrate the reduction of staleness in Figure~\ref{fig:uplink-design}.
In Figure~\ref{fig:uplink-design:no-uplink}, we do not use the uplink capacity available on the satellite.
Thus, the satellite can only access images captured by itself, which is Oct 5, Oct 15 and Oct 25.
Thus, the reference image for Oct 15 will be Oct 5, result in a staleness of 10 days.
As the image captured at Oct 15 cannot be used as reference image due to the cloud in the image, the satellite will still use original reference image (Oct 5) for the new incoming reference image (Oct 25), resulting in a staleness of 20 days. \jc{i like this example, except the part about the cloud. i understand under your current technique or some reference implementation, such cloudy images will be discarded, but a smart baseline can always utilize the non-cloudy part, so reviewers may still argue that most of the Oct-15 image can be used without using the uplink. my suggestion is to simply assume the latest reference image in (a) is 20 days ago (or some big staleness), and the latest ref in (b) is only 2 days ago (or some small staleness), and don't use cloudy images.}
Thus, the average staleness of reference images in this example is 15 days.
In Figure~\ref{fig:uplink-design:with-uplink}, we use the uplink of the satellites to provide the satellite up-to-date reference images from other satellites.
This allows the satellite to use image captured at Oct 10 as reference image for Oct 15, and Oct 20 as reference for Oct 25, reducing the average staleness of reference image to only 5 days.






% In contrast to letting the satellite handle the reference images, our \textit{uplink-based} design empowers the satellite to 
% % \item \textit{Store minimally compressed references with limited space:} By uploading images, the satellite stores references solely for a \textit{small subset of locations} it will pass over before ground contact.\end{packeditemize}
% use the images from other satellites as the reference, and thus significantly reduces the staleness of the reference image.

\mypara{Measure the potential}
To further quantify how much our \textit{uplink-based design} reduces the staleness of reference images, we use the satellite images from Washington area in Sentinel-2 dataset at year 2020, and compare the average staleness of reference images between our uplink-based design and traditional satellite-local design.
We found that by leveraging uplink, the staleness of reference images is reduced by half.
This reduction will be more significant if there were more satellites in Sentinel-2 (currently only 2 satellites).
\jc{with only two satellites, this example will probably weaken your argument. i thought there was another potential dataset (though you probably don't have the full data from it?) which has a much bigger set of satellites, right? it's totally ok to motivate your solution using a dataset that you won't use in your eval, especially since it's not open to the public. you can use that as the first example, and then bring up sentinel-2}




\mypara{An alternative}
An alternative way of allowing the satellite to access images from other satellites is by leveraging inter-satellite links.
However, unlike the satellite designed for internet access, earth observation satellites typically do not have such inter-satellite link capacity.
In contrast, our design is based on the uplink capacity, which is readily available on existing satellites.




\subsection{\name: workflow}

\begin{figure}
    \includegraphics*[width=1\columnwidth]{figures/earth-satellite.pdf}
    \caption{\name uploads the reference images to the satellite and use these images to calculate, encode and download the changes.}
    \label{fig:uplink-workflow}
\end{figure}


We introduce \name, a system that updates the reference images using uplink.
The workflow of \name is illustrated in Figure~\ref{fig:uplink-workflow}. Specifically,
\begin{packeditemize}
\item During ground contact, images for upcoming fly-by locations before the next ground contact are uploaded to the satellite.
\item When passing over a location, the satellite captures and encodes changes using the corresponding reference image.
\item During the next ground contact, the ground downloads the changes from the satellite.
\end{packeditemize}



\subsection{Challenge: limited uplink capacity}


The above workflow leverages \textit{uplink} to upload the reference images to the satellite.
However, as illustrated in \S\ref{subsec:satellite-connectivity}, the satellite uplink is extremely limited compared to the downlink capacity, as it is mainly used to send control messages rather than streaming imageries.
Thus, the main challenge of \name is to handle limited uplink bandwidth.

To reduce the uplink capacity, we develop two techniques:
\begin{packeditemize}
    \item \textbf{\textit{Low-resolution reference}}:
    Stream low-resolution reference image through uplink and detect changes using such low-resolution reference.
    The key insight is that: under high-resolution imagery, the geographical changes on the earth typically corresponds to a large area on the earth.
    These changes can thus be detected even using low-resolution image.
    \item \textbf{\textit{Cloud-free image as reference}}:
    \name uses cloud-free images as the reference, and update the on-board reference only when \textit{other} satellite obtains a new cloud-free image.
    This allows \name to further reduce the frequency of updating the reference image.
    Note that one can potentially leverage the cloud-free areas in a cloudy images to further update the reference images, \name leaves this solution to future work.
\end{packeditemize}






% on reference images, we conduct a back-of-the-envelope measurement using the specification of a DOVEs constellation satellite~\cite{dove-constellation}. 
% This satellite contains 720GB storage space\kt{need more specs here}. We assume reliable uplink during ground contact with ample bandwidth (real uplink conditions discussed in \S\ref{subsec:upload-reference-policy}). 
% We show that:
% \begin{packeditemize}
% \item The reference image needs to be compressed by a factor of 20, while the reference images need to be compressed by a factor of 500 if reference images are stored and updated by the satellite itself.
% \item For a given location, the satellite can use images older than 90 minutes as the reference image. In contrast, the satellite can only use images older than 10 days as the reference (as the satellite.
% \end{packeditemize}








% We point out three concrete potentials achieved by these benefits.
% First, if 



% Prior work fails to realize the potential of change-based encoding due to storing reference images for all geographical locations on-board.

% We observe that,  for a given geographical location, its corresponding reference image only needs to be on-board when the
% satellite flies by that location. In other word, instead of saving
% the reference images for all locations, 
% that the satellite is going to fly by.


% \mypara{Workflow} The workflow is described as follows:
% \begin{packeditemize}
%     \item During current ground contact: the ground upload reference images for locations before next ground contact.
%     \item Before next ground contact: the satellite photos the earth and only encode the changes
%     \item During next ground contact: the satellite send the encoded changes to the ground.
% \end{packeditemize}




% \mypara{Advantage} Compared to storing the reference images of all locations on-board, our uplink-based design provides two advantages:
% \begin{packeditemize}
%     \item This design allows the satellite to access a higher-quality reference image under limited satellite storage.
%     \item This design allows the satellite to use images from other satellites as the reference. 
% \end{packeditemize}
% We will show the practical benefit of these two advantages in \S\ref{??}.







% \section{Overview of \name}

% \jc{we should merge 3 and 4. the uplink-based workflow is basically the workflow of earth+, right?
% }

% We introduce \name, a system that grants the satellite access to fresh reference images from other satellites using uplink capabilities.
% By having fresh reference images on-board, \name allows the satellite to download much less changes without sacrificing the quality of downloaded images.

% \name faces two practical challenges:

% \jc{the second challenge is more relevant to your ``uplink'' idea. we should elevate it. change detection and illumination alignment are critical for your solution to be functional, but they are definitely secondary as a contribution (unless i totally misunderstood).}

% \jc{correspondingly, 4.1 should be moved to after sec 5. in fact, i'd STRONGLY recommend that you do NOT explain the solution for cloud and illumination alignment until AFTER section 5. So everything before the end of section 5 will assume that there is NO cloud and NO need for illumination alignment. so people can FOCUS on your idea of uplink!}

% \begin{packeditemize}
% \item Accurately detect changes amidst cloud cover and varying illumination, all while using limited computational resources of the satellite.
% \item Maintaining a fresh reference image on-board within the constraints of the limited uplink capacity and storage space on the satellite.
% \end{packeditemize}

% \jc{before we dive into details, can this section highlight some key insight/ideas that enable us to address the key challenges?}


% We will briefly introduces the workflow that \name uses to handle these two challenges, and delve into these challenges in detail in the following sections.






% % We propose \name, a concrete system that leverages uplink to maintain fresh reference images on-board so that minimum amount changes need to be downloaded from the satellite.


% % The key practical challenge of \name is two-fold:
% % \begin{packeditemize}
% %     \item Accurately detect changes with the disturbance of cloud and illumination condition using limited computation resources on the satellite.  
% %     \item Frequently update the reference images using extremely limited uplink capacity, while sticking within the available storage space on the satellite.
% % \end{packeditemize}

% % We will overview these two challenges, and then discuss how \name addresses these two challenges in future sections.





% % Different from traditional change-based compression that assumes two consecutive images are similar (\textit{e.g.} video compression), two consecutive observations for the same location may be very different due to their different \textit{dynamism}, as shown in Figure~\ref{fig:satellite-imagery-dynamism}.
% % % We can see that these two images differ significantly due to the dynamism in satellite imagery.
% % In \name, we focus on handling the two most significant sources of dynamism: cloud and illumination.
% % Note that while there are also other sources of dynamisms (\textit{e.g.} sensor noises and geographical misalignment), \name does not explicitly handle them since these dynamisms only appear in raw satellite imagery (\textit{i.e.} Level-0 satellite imagery product), which is not available in public dataset.


% % \mypara{Limited on-board storage and computation}
% % The computation and storage on the satellite are limited.


% % \mypara{Limited uplink and downlink bandwidth}
% % The uplink and downlink bandwidth are limited.







% \subsection{Detecting changes in satellite imagery}


% \begin{figure*}
% \centering
% \includegraphics[width=1.5\columnwidth]{figures/earth_plus_pipeline.pdf}
% \caption{Overview of Earth+ architecture. Earth+ upload reference images to the satellite, then the satellite photo the earth and calculate changes. The satellite then stream the changes down to the earth.}
% \label{fig:earth-plus-pipeline}
% \end{figure*}




% \subsection{Refresh reference image using limited uplink}

% In satellite scenario, uplink is really limited.

% \name stores the reference images on-board, and use uplink to update images when the reference images get stale.




% This is an operation that are widely employed
% However, \name remains applicable to a wide range of applications where cloudy data holds less significance (\textit{e.g.} road detection, agriculture monitoring).

% \mypara{Ground contact phase} During this phase, the ground station uploads reference images to the satellite and retrieves encoded changes from the satellite.





% The workflow of \name contains two phases: ground contact phase and image capturing phase.

% \mypara{Image capturing phase} During image capturing phase, \name handles the dynamism of satellite imagery and detects changes in the captured image using the following steps:
% \begin{packedenumerate}
%     \item The satellite runs a cloud detection model that returns a probability for each pixel indicating how likely this pixel being cloudy (the detail in \S\ref{??}).
%     \item The satellite aligns the illumination of observed image to the reference image.
%     Note that we only align illumination on highly noncloudy areas (cloud probability < 0.2) to avoid letting our estimated illumination condition biased by the highly-reflective cloudy areas.
%     \item The satellite calculates and encodes the changes on areas that are non-cloudy. Other areas (including cloudy areas) will not be encoded.
% \end{packedenumerate}

% The above pipeline discards cloudy data, which is not desirable for applications like weather forecasting.
% However, \name can be still applied to a wide set of applications in which cloudy data are of less value (\textit{e.g.} road detection, agriculture monitoring).


% \mypara{Ground contact phase} During ground contact phase, the ground station upload the reference images to the satellite, and download the encoded changes to the ground.



% \subsection{Benefit of uplink-based design on \name}



% The uplink-based design allows the reference images to be less compressed and more up-to-date.
% This provides three concrete benefits when compressing satellite imagery:
% \begin{packeditemize}
%     \item \textit{Less data need to be downloaded under the same amount of change} by using a high-quality reference image.
%     \item \textit{Less changes compared to the reference} since the reference image is more up-to-date.
%     \item \textit{Accurate cloud detection under limited compute} by using a high-quality reference image as the \textit{extra} input.
% \end{packeditemize}


% By implementing the uplink-based design, the reference images of \name are less compressed and more up-to-date, leading to three specific advantages:
% \begin{itemize}
% \item \textit{Reduced change relative to reference image:} Leveraging up-to-date references diminishes differences.
% \item \textit{Enhanced change detection accuracy:} Superior reference image quality aids precise detection.
% \item \textit{Computationally-efficient cloud detection:} Utilizing high-quality reference images as supplementary input allows \name to accurately detect clouds using a cost-effective detection model.
% \end{itemize}

% These advantages enable \name to minimize per-image data downloads and alleviate satellite resource requirements. Quantitative assessment of these benefits will be conducted in our evaluation.

% By instantiating the uplink-based design, the reference images of \name are less compressed and more up-to-date. This brings \name three concrete benefits:
% \begin{packeditemize}
% \item \textit{Less changes compared to the reference image} by using up-to-date reference image.
% \item \textit{Accurate change detection} by using high-quality reference image.
% \item \textit{Cheap cloud detection} using the high-quality reference image as the extra input to the cloud detector.
% \end{packeditemize}
% These benefits allow \name to download less data per image and reduce the resource demand on the satellite. 
% We will quantitatively measure these benefits in our evaluation.

% \kt{Should we measure these benefits here, or later in the evaluation? I feel like here we should put the benefit into the context of performance metrics (like PSNR / downloaded data), but these benefits are difficult to measure without specifying which algorithm we are using}




% \subsection{Practical challenges}




% The technical challenges of \name are three-fold.

% First, on the satellite, how to reduce the cost of cloud detection and change detection so that they do not exceed the limited on-board computation capacity while still being accurate?


% Second, on the ground, how to obtain a cloud-free reference image for a location (\S\ref{??})?
% This is challenging because there can be no recent images of a given location that are completely cloud-free.
% For example, Seattle can be partially cloudy for months during winter.

% Third, on the ground, how to determine the locations and the quality of reference images that need to be sent to the satellite \S\ref{??}?
% This is challenging since the uplink capacity can vary significantly between different ground contacts.


% The design challenges of \name is three-fold:
% \begin{packeditemize}
%     \item How to obtain the reference images fro a designated geographical location, given that recent images of that location may all be cloudy?
%     \item How to determine the locations and the quality of reference images before sending them to the satellites?
%     This is challenging since the total size of the reference images need to fit into the uplink capacity, which is limited and sometimes even unavailable (characterized in \S\ref{??}).
%     \item How to perform change-based encoding under varying cloud and illumination conditions, using limited computation on-board?
% \end{packeditemize}







% \subsection{Benefits}
% \begin{outline}


%     \1 Benefits 1. Significantly reduced storage demand
%     \2 Figure~\ref{fig:storage-vs-downlink} to compare between different solutions
%     \2 Dimension 1: Storage demand
%     \3 If the satellite keep all reference images on itself --> 10-days worth of image
%     \3 If the ground stream the reference image to the satellite --> 90-minutes worth of image (ground-contact time), 160x reduction on the filesize of reference image need to be stored, much less.
%     \2 Dimension 2: daily generated data
%     \3 Traditional satellite store all areas.
%     \3 Earth+ only store changed areas on the satellite ==> much smaller file size.

%     \1 Benefit 2: Reduce change by referring to newer images on other satellite
%     \2 Figure~\ref{fig:multi-satellite-as-reference} to show the potential of using multiple satellites.
%     \2 Takeaway: 2x less changed areas when using images from 2 satellites as reference.
% \end{outline}












% \begin{packeditemize}
% \item Significantly reduce the storage demand on the satellite
% \item The satellite can virtually have access to the latest images from other satellites --> much less changes 
% \item The ground can timely configure the encoding hyperparameters.
% \end{packeditemize}



% \subsection{Techinical challenges}

% \kt{functional satellite}
% \kt{Multiple satellites}

% \begin{outline}
% \1 On the satellite
% \2 Detect changes using the reference image, given that the cloud conditions and illumination conditions are constantly changing.
% \2 Fit into the limited resource (in terms of computation and on-board storage) of the satellite.
% % \2 Handling cloud and detect changes using limited on-board resource. 
% % \3 Background: Cloud detection can be difficult and computation-demanding. Example: very difficult to distinguish between snow and cloud merely from the pixel value.
% % \3 Challenging: Accurate cloud detection is expensive (e.g. neural-network-based cloud classification). Need some citations. Ideally with some quantitative numbers.
% \1 On the ground
% % \kt{How to use uplink efficiently}
% % \kt{handle limited uplink}
% % \kt{handle limited availability of uplink}
% % \kt{having up-to-date reference}
% % \kt{Heterogeneity between different locations}

% \2 How to create reference image from multiple images observed by multiple satellite? 
% \3 Challenging: Latest image may be cloudy, and the latest non-cloudy image may be too old (eg during winter period, an area can be always cloudy for months).
% \2 How to handle the case when the uplink is unavailable or of low bandwidth?
% % \2 How to customize the hyperparameters (HPs) with minimum computation overhead?\jc{this comes out of nowhere. there's nothing about this in the last section}
% % \3 Challenging: optimal HPs vary across locations. e.g. water area v.s. forest area. 
% % \4 Water area --> can detect change in a very low resolution and still get accurate results.
% % \3 Forest area --> change is often subtle, need to detect change in a very high resolution 
% % \3 Challenging: optimal HPs vary across time in the year. e.g. harvesting season changes much more frequently than non-harvesting season.

% \jc{another natural challenge is how to minimize the uplink bandwidth demand. any reason this is not mentioned? }
% \end{outline}



% \begin{figure}
% \includegraphics[width=1\columnwidth]{figures/satellite-pipeline.jpg}
% \caption{The pipeline on the satellite}
% \label{fig:satellite-pipeline}
% \end{figure}












% \section{Communicating with the satellite}

% \subsection{Downloading}

% Existing satellites download images in their entirety for the locations that the satellite passes by.
% Different from this, \name downloads the changes, together with the illumination information required for reconstructing the unchanged areas on the ground.

% \subsection{Uploading}

% During each ground contact, \name needs to upload the changed areas of the reference images to the satellite.

% \mypara{Prior API} Prior work communicates with the satellite through the following API:
% $$
% image = download(location)
% $$

% We change this API to
% % $$
% change, illum = download(location) \\
% $$


% \begin{outline}
%     \1 Workflow on the satellite
%     \1 Uploading reference image
% \end{outline}






\section{Uploading reference to the satellite}


\name stores the reference images on-board the satellite and updates them using the uplink.
This section discusses how \name stores the reference images on the satellite and update them while sticking into limited uplink capacity and  on-board storage.





\subsection{Uplink is limited}
% As the downlink of the satellite is 200 Mbps, 800$\times$ larger than the uplink (250 kbps). As a result, the compression ratio of reference image
% allocate 15 GB to store the references, and the remaining 15 GB to store the changes.
% This is based on the 

% \name stores the reference images of these $70k$ locations on-board.
% As the satellite stores the reference image on-board, 
% As the satellite restarts its orbit  one location once per 10 days~\cite{sentinel-2-revisit} and has about 7 times ground contact per day, it means that the satellite needs to download 1050 GB images 

% As a result, if the satellite can download $k$ images during each ground contact, the satellite then downloads $70k$ images during 10 days, where \name stores the reference of $70k$ images on-board.



% \mypara{Anchor}
% \name estimates the compression ratio of reference images, compared to downloading them into uniform quality.

% \mypara{Storaging reference images}


As illustrated in \S\ref{subsec:satellite-connectivity}, the uplink capacity of the satellite is much more limited compared to the downlink capacity since the uplink is only used to send control messages.
To put this into context, we analyze the demand and the supply ouse DOVEs constellation as an example.
During each ground contact, the ground can download data from the satellite at a rate of 
During each ground contact, the ground can send the data to the satellite at a rate of 250kbps~\cite{dove-uplink-downlink} for 10 minutes, which only allows uploading about 19 MB data in total.
While this is enough for the ground to send its control messages, it only allows one to update the reference image for about 5$km^2$ areas in its entirety.
In contrast, the downlink downloads about 4000 $km^2$ images in total each time.



\begin{figure}
    \centering
    \includegraphics[width=.9\columnwidth]{figures/placeholder-reference-compression.pdf}
    \caption{Compressing reference image using resolution instead of bpp allows \name to download fewer areas while still detecting changes.}
    \label{fig:reference-compression}
\end{figure}





\subsection{Lowering the resolution}


In order to handle limited downlinks, \name uploads \textit{compressed} reference images to the satellite.
While compressing the reference image, our insight is that
One is by lowering the image resolution so that less amount of pixels will be included in each image.
The other one is to assign fewer bits to each pixel (\ie less bits-per-pixel), which reduces the file size of the image at the cost of less accurate pixel values.
We found that lowering the resolution allows \name to detect changes more accurately compared to lowering the bits per pixel.
This is because that the change on the satellite is at a large scale (\eg in harvesting season, the harvesting happens over the whole farm, where a typical 1$km^2$ farm corresponds to a 300$\times$300 pixel block in the image), so these changes are still visible even under a low resolution.
However, the pixel value change can be small (\eg watering a farm only causes the soil to be slightly darker).
As a result, the pixel value need to be accurate in order to identify these small changes, thus a high bit-per-pixel is required.



To further support this point, we perform a measurement to see how much the change detection accuracy (measured in F1 score) varies with respect to lowering the resolution and lowering the bit-per-pixel.
As shown in Figure~\ref{fig:reference-compression}, we can see that under the same file size, the change detection accuracy of lowering the resolution is siginificantly higher than lowering the bit-per-pixel.



\subsection{Storing the reference image on-board}


To further save the uplink usage, \name stores the low-resolution reference image on-board for all geographical locations in the satellite storage. (We will discuss how to determine the resolution of reference images in \S\ref{??}).



\kt{Figure out a way to say the benefit.}

Because \name stores only the changed areas on-board, squeezing out spaces for storing the reference images.
To make sure that the storage reference image does not exceed the bandwidth budget, we leverage the following two observations:
\begin{packeditemize}
    \item 
\end{packeditemize}


With this optimization, \name further reduces the demand of uplink by 4$\times$, allowing \name to upload the reference images using limited uplink (see Figure~\ref{??} for detailed evaluation).



\mypara{Updating policy}








\subsection{Determining the resolution of reference image}


\kt{TBD}.




% \mypara{Compression ratio for reference}
% We first estimate the compression ratio required for the reference images in order to store them on-board.
% During each ground contact, the satellite can download 15 GB images.
% Assume these 15 GB images corresponds to $k$ geographical locations.
% As the satellite contacts to the ground 7 times per day and revisits the same location in 10 times, it means that the satellite has at most $70k$ distinct geographical locations to handle, corresponding to $1050$ GB worth of images.


% We assume that the satellite has 30 GB storage\footnote{}.
% We allocate half of the storage space ($\ie$ 15 GB) to store the reference images, resulting an 70$\times$ compression ratio.

% Note that this solution assumes that \name can store the downloaded images using only half of the storage space, which is true for \name as \name only stores the changed areas rather than the whole images for future downloading.



























\section{On-board change detection}



\begin{figure}[ht]
    \includegraphics[width=.99\columnwidth]{figures/dynamism.pdf}
    \caption{Two consecutively-captured satellite imagery have similar content on the ground but can significantly differs in terms of pixel value due to cloud and illumination difference.}
    \label{fig:satellite-imagery-dynamism}
\end{figure}
    



\subsection{Background}
Change detection in image sequences has been widely studied, especially in video codec literatures (\eg H.264~\cite{h264}).
This approach works well when two consecutive images have a small pixel value difference.
However, in satellite imagery, this pixel difference can be extremely large, even when their geographical content is almost identical.
This is because that the time gap between two consecutively-captured image for one geographical location is typically several days (\eg 1 day for Planet~\cite{planet} and 5 days in Sentinel-2~\cite{sentinel-2-revisit}).
As a result, the illumination condition and the cloud condition can vary a lot.
For example, in two consecutively captured images shown in Figure~\ref{fig:satellite-imagery-dynamism}, these two images have almost identical geographical content but pixel-value-wise these two images still differs a lot due to cloud and illumination difference\footnote{Note that there are other potential sources (\textit{e.g.} sensor noise, image misalignment) that can triggers large pixel difference. \name does not explicitly address them, as they pertain to raw satellite imagery (\textit{i.e.} Level-0 satellite imagery product), which is not accessible in public datasets.}

To handle cloud and illumination difference in satellite imagery, \name employs the following workflow for change detection.



\subsection{Change detection workflow of \name}
\begin{packeditemize}
    \item Cloud removal: detect \textit{\textbf{highly-cloudy}} areas in the satellite imagery using decision tree classifier, and remove this part of the data (by filling the corresponding pixels with zero pixel value).
    \item Illumination alignment: align the illumination between the reference image and the captured image on less-cloudy areas using linear regression.
    \item Change detection: inside those less-cloudy areas, mark the pixels that has high pixel difference compared to the reference images as changed.
    \item Encoding: encode the changed pixels via existing image codecs.
\end{packeditemize}
% involves two phases: the ground contact phase and the image capturing phase.
% \begin{packeditemize}
% \item \textit{When contacting the ground}, the satellite downloads the changes for previously visited locations and updates the reference images for future locations (detailed reference image updating policy shown in \S\ref{??}).
% \item \textit{After capturing a image} for a geographical location, \name runs a cloud detector to remove clouds and aligns the illumination of captured image and the reference image. \name then detects changed areas and encodes the changed areas.
% % The satellite runs a cloud detection model that assigns cloud probabilities to pixels (details in \S\ref{subsec:cloud-detector}).
% % \item Aligning the illumination on the ground areas with the reference image.
% % \item Computing and encoding changes for non-cloudy regions. The data of cloudy areas will be discarded.
% \end{packeditemize}

Note that the abovementioned pipeline removes those pixels that are highly cloudy.
Acknowledging that this makes \name less applicable in cloud-sensitive applications like weather forecasting, 
we argue that a wide range of applications (\eg autonomous road detection, agriculture monitoring, etc) will filter out cloud data as they are focusing on the geographical content on the ground rather than cloud.


We highlight that this workflow is computationally efficient.
We will illustrate why this workflow can stick with desired accuracy in \S\ref{??}.



% \subsection{Workflow}

% \begin{outline}
% \1 To detect change under varying cloud and illumination condition, \name use the following workflow on the satellite (Figure~\ref{fig:satellite-pipeline}).
%     \2 Cloud detection \& removal (assuming the cloud data can be discarded)
%     \2 Illumination alignment (we use a simple linear regression algorithm to determine the lighting change).
%     \jc{both alignment and cloud detection/removal come out of blue. downplay them if we don't touch the cloud/alignment-related stuff at all, to avoid confusion. if we touch them, please motivate the change in section 2 and 3 first.}
%     \kt{I motivated this challenge in section 3. I think it should not appear in section 2 as it is not a design question but rather an implementation question.}
%     \2 Change detection
%     \2 Encode and store the changes
% \end{outline}















\subsection{Compute-efficient cloud detection}
\label{subsec:cloud-detector}



\begin{table}[]
\footnotesize
\begin{tabular}{|l|l|l|l|}
\hline
& \begin{tabular}[c]{@{}l@{}}Computation\\ cost\end{tabular} & \begin{tabular}[c]{@{}l@{}}Correctly \\ classified pixels\end{tabular} & \begin{tabular}[c]{@{}l@{}}Accuracy\\ (IoU)\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Inaccurate cloud detector\\ (decision-tree-based)\end{tabular} & 0.01 GFlops                                                & 96\%                                                                   & 0.5                                                                      \\ \hline
\begin{tabular}[c]{@{}l@{}}Accurate cloud detector\\ (neural-network-based)\end{tabular}  & 1000 GFlops                                                & 99\%                                                                   & 0.9                                                                      \\ \hline
\end{tabular}
\caption{A cheap cloud detector can still correctly classify over 96\% of the geographical areas.}
\label{tab:inaccurate-cloud-detector}
\end{table}


On the satellite, the most computationally intensive task within \name is cloud detection. Previous research~\cite{??} demonstrates that achieving accurate cloud detection involves neural networks with tens of layers, significantly exceeding the computational budget on the satellite.

To address this challenge, \name employs two observations.

First, by incorporating a cloud-free reference image as an auxiliary input, the cloud detector achieves comparable accuracy with much less computation. 
This is enabled by allowing the cloud detection algorithm to analyze pixel changes between the current image and the reference.
This approach is particularly effective in cloud detection, where clouds induce substantial pixel changes in comparison to the reference image.

Second, while a compute-intensive cloud detector accurately handles complex scenarios (e.g., faint haze and cloud edges), these instances constitute only a small portion (around 4\%) of the observed satellite imagery.
\kt{we need a measurement here}

Building on these insights, \name employs a pixel-value-based decision tree to assign a cloud probability to each pixel. This tree takes both the observed and reference image pixel values as the input. 
Additionally, \name runs the decision tree using the downsampled image (16x downsampled, width and height) as the input, as the JPEG-2000 codec uses a minimum block size of 16.



To account for potential prediction errors from our cheap cloud detector, we make slight alterations to the illumination alignment~\ref{subsec:illumination-alignment} and change detection~\ref{subsec:change-detection} of \name, with the assumption that cloud detection errors commonly occur around a predicted cloudy probability of 0.5. 
This property holds as our cloud detector uses decision tree algorithm, which generates a cloud probability near 0.5 when those pixels with similar pixel values in the training set are approximately half cloudy and half non-cloudy.



% On the satellite, the most computational expensive task of \name is the cloud detection.
% As prior work shows [??], it requires tens of layers of neural network to perform accurate cloud detection, which significantly exceeds the computation budget of the satellite.

% To handle this challenge, \name makes two observations.

% First, we observe that by the cloud detector can comparable accuracy while demanding significantly less computation power by introducing a cloud-free reference image as an auxiliary input.
% This is because the cloud creates a huge pixel change on the images, and the cloud detector can easily detect such pixel change using the reference image. 


% Second, though compute-demanding cloud detector can accurately detect cloud in intricate cases (\textit{e.g.} light haze and the boundary of the cloud), these cases only account for a small fraction (roughly 4\%) of the observed satellite imagery.




% Based on these observations, \name assigns a cloud probability to each pixel by running a pixel-value-based decision tree using the pixel value of both the reference image and the observed image.
% To further reduce the computation cost, \name runs the cloud detector on a image that are downsampled 4x on both width and height.



\subsection{Illumination alignment}
\label{subsec:illumination-alignment}

Let $\mathbf{R}$ represents the reference image, $\mathbf{C}$ represents the current image. As shown in ~\cite{illumination-model}, on cloud-free areas, we have $\mathbf{C}=k\mathbf{R}+d$, where $k$ and $d$ is two constants that do not change between different areas in the current image. To obtain these two constants, \name runs standard linear regression on areas confidently identified as non-cloudy (cloud probability less than a fixed constant $\alpha=0.2$).



% \subsection{Handling cloud detection errors}

% % We first categorize the error of cloud detector into two types:
% % \begin{packedenumerate}
% %     \item Boundary error
% %     \item Confusion error
% % \end{packedenumerate}



% First, as the illumination alignment and change detection relies on cloud detection results, we run these algorithms \textit{conservatively} so that potential cloud detection errors will be accounted as changes. 
% Concretely, during illumination alignment, . This approach ensures that cloudy pixels do not influence illumination alignment.





\subsection{Change detection}
\label{subsec:change-detection}

\name detects changes by partitioning the current image and the observed image to 16x16 blocks, calculating the average pixel difference between the observed image and the reference image in each block, and then marking those blocks with average pixel difference greater than a threshold $\theta$ as changed.
Note that \name does not download those changes that are confidently caused by cloud (defined as those changes with cloud probabilities exceeding $\beta=0.8$).


We calculate the changes in each 16x16 block as the current satellite encoding algorithm (\textit{i.e.} JPEG-2000) encodes the images block-by-block and the minimum size of each block is 16x16.





% As our cheap cloud detector may generate the wrong prediction, we handle this prediction error using the following policy:
% \begin{packeditemize}
%     \item When aligning illumination, \name operates on areas that are certainly non-cloudy (cloud probability smaller than a constant $\alpha=0.2$).
%     This allows \name to align the illumination on the ground without being affected by cloudy pixels.
%     \item When detecting changes, \name only eliminates those areas that are certainly cloudy, defined as those areas with cloud probability greater than $1-\alpha$.
% \end{packeditemize}

% Note that the policy above assumes that the cloud detection makes error when the predicted cloudy probability is close to 0.5.
% This is true for our cloud detector as our cloud detector leverages decision tree algorithm, which generates the predicted probability by directly counting the number of cloudy observations (under the current decision) and the number of non-cloudy observations.


% Selective Accuracy: The examination of cloud occurrences highlights that intricate cases, such as those involving light haze and water reflection, account for a mere fraction of the satellite's coverage (roughly 4\%). Conversely, a less sophisticated cloud detector achieves accurate cloud detection in over 96\% of the observed area. Thus, the high-cost cloud detector's advantages are mainly relevant to a minimal subset of circumstances.


% Informed Detection: Leveraging a cost-effective cloud detector as its backbone, \name capitalizes on the reference image to augment detection capabilities. By judiciously combining these resources, we strike a balance between accuracy and computational efficiency.




\subsection{Encoding the changes}


\name aims to downloads the detected changes with a fixed encoding quality.
This fixed quality is decided by a parameter $b$, where $b$ describes the file size divided by the number of pixels of changed areas (\ie bit-per-pixel on changed areas).

As a result, \name uses the region-of-interest encoding feature of an JPEG-2000 encoder (Kakadu~\cite{kakadu}) while constraining the encoded file size to be $b$ times the number of changed pixels.

% The region-of-interest encoding of Kakadu accepts a parameter $b'$ that describes the file size divided by the amount of pixels of all areas.
% As a result, we let $b' = b \times \frac{\text{\# of changed pixels}}{\text{\# of all pixels}}$ 



\subsection{Reconstructing the image on the ground}

As \name only download the changed areas, \name reconstructs the changed areas by using $k\mathbf{R}+d$, where $k$ and $d$ are the two illumination alignment constants downloaded from the saatellite, and $R$ is the reference image.




\subsection{Downloading images for future reference}


\name will download the current images in its entirety and use it to substitute the reference image of the same location if:
\begin{packeditemize}
    \item The current image does not contain much cloud (defined as the fraction of cloudy pixels is smaller than $x\%$, where \name uses $x=0.5$ by default).
    \item The corresponding reference image is stale (\textit{i.e.} the time delta between the reference image andthe current image is more than $k$ months old, we use $k=1$ by default).
\end{packeditemize}
Note that we download the current image with a encoding quality $b_{0}$ higher than the quality $b$ used to encode the changes, as the current image will be used multiple times to reconstruct all future images (until a new reference image is obtained).





% \kt{Goal: nuggets, reference image quality, resolution v.s. change detection threshold change-by region; if a change is missed, safe-guarding mechanism to save this missed change?}
% \kt{Uplink quality is too low --> can satellite realize that the quality is too low? Random fix?}

% \kt{Why uplink is small? Reason 1: every location --> lowest resolution: rightly fit the predicted spatial granularity of change}
% \kt{If the prediction is wrong, we have someway to detect it: periodically better resolution and see if the detection is better}
% \kt{End-to-end evaluation}
% \kt{Measurement: a very }





% \subsection{Safeguarding potential errors}

% \begin{outline}
% \1 The cheap cloud detector of \name may still generate errors.
% \1 We categorize 
% \1 To safeguard against such errors, we provide two mechanisms.
% \1 Safeguard mechanism 1: when in doubt if an area is cloudy / changed, just download that area.
%     \2 Concretely, \name will have 
% \1 Safeguard mechanism 2: when an area is not downloaded for e.g. 2 months, download it regardless of its cloud condition.
% \end{outline}


% \begin{packeditemize}
% \item Cloud removal
% \item Need to mention the assumption that cloudy data are not useful (this need to be justified much earlier)
% \item Illumination alignment
% \item Change detection
% \item Encoding
% \end{packeditemize}


% \subsection{Incoporating resource constraint on the satellite}

% \begin{packeditemize}
% \item Save compute: decision-tree-based cloud detector on the downsampled satellite image.
% \item Save storage: downsampled version of the reference image.
% \item Errors WILL occur. Error handling policy: when in doubt, just download.
% \end{packeditemize}


% \subsection{Handling subtle but consistent change}

% \begin{packeditemize}
%     \item Guarantee that each area WILL be downloaded once every X months.
% \end{packeditemize}





